Sampling-Based Query Re-Optimization

Despite of decades of work, query optimizers still make mistakes on "difficult" queries because of bad cardinality estimates, often due to the interaction of multiple predicates and correlations in the data. In this paper, we propose a low-cost post-processing step that can take a plan produced by the optimizer, detect when it is likely to have made such a mistake, and take steps to fix it. Specifically, our solution is a sampling-based iterative procedure that requires almost no changes to the original query optimizer or query evaluation mechanism of the system. We show that this indeed imposes low overhead and catches cases where three widely used optimizers (PostgreSQL and two commercial systems) make large errors.

==> abstract.tex <==
\begin{abstract}
Query optimizers rely on reasonable cardinality estimates to generate good query plans.
Unfortunately, histogram-based cardinality estimation approaches often fail to detect the dependency presented in the data,
which could lead to poor cardinality estimates.
On the other hand, sampling-based cardinality estimation can usually provide more accurate cardinality estimates on correlated data.
However, sampling incurs additional overhead and cannot afford to be used for every candidate plan considered by the optimizer.
In this paper, we study an iterative sampling-based query re-optimization procedure that can be viewed as a compromise between these two extremes: pure histogram-based and pure sampling-based query optimization.
In each round of iteration, we use sampling to refine cardinality estimates of the optimal plan returned by the optimizer, and invoke the optimizer again by feeding it with the refined cardinality estimates.
We repeat doing this until the optimal plan is fixed.
We further study this re-optimization procedure in detail, both theoretically and experimentally.
Our theoretical analysis suggests that the efficiency of this procedure and the quality of the final plan returned can be guaranteed under certain assumptions, and our experimental evaluation on the TPC-H benchmark database as well as our own benchmark with highly correlated data demonstrates the effectiveness of this approach.
\end{abstract} 

==> abstractNew.tex <==
\begin{abstract}
%Query optimizers rely on reasonable cardinality estimates to generate good query plans.
%Unfortunately, histogram-based cardinality estimation approaches often fail to detect the dependency presented in the data,
%which could lead to poor cardinality estimates.
%On the other hand, sampling-based cardinality estimation can usually provide more accurate cardinality estimates on correlated data.
%However, sampling incurs additional overhead and cannot afford to be used for every candidate plan considered by the optimizer.
%In this paper, we study an iterative sampling-based query re-optimization procedure that can be viewed as a compromise between these two extremes: pure histogram-based and pure sampling-based query optimization.
%In each round of iteration, we use sampling to refine cardinality estimates of the optimal plan returned by the optimizer, and invoke the optimizer again by feeding it with the refined cardinality estimates.
%We repeat doing this until the optimal plan is fixed.
%We further study this re-optimization procedure in detail, both theoretically and experimentally.
%Our theoretical analysis suggests that the efficiency of this procedure and the quality of the final plan returned can be guaranteed under certain assumptions, and our experimental evaluation on the TPC-H benchmark database as well as our own benchmark with highly correlated data demonstrates the effectiveness of this approach.

%Query optimizers rely on reasonable cardinality estimates to generate good query plans.
%Sampling-based approaches can provide more accurate cardinality estimates than histogram-based approaches used by current query optimizers, especially on correlated data.
%However, sampling also incurs higher overhead and cannot afford to be used for every candidate plan considered by the optimizer.
We study how to exploit the power of sampling in query optimization without significantly increasing optimization time. Rather than using sampling during the search for an optimal plan, we use sampling as a post-processing step after the optimizer has finished its search to validate cardinality estimates for the final plan chosen by the optimizer.
%If there were significant errors, we give the optimizer second chance to generate a better plan.
%Specifically, we propose an iterative procedure.
%%that can be viewed as a compromise between pure histogram-based and pure sampling-based query optimization:
%%we use sampling as a validation step to catch cardinality estimation errors in the final plan chosen by the
%%optimizer, and give the optimizer second chance to generate a better plan if the errors were significant.
%%This can help us avoid disastrous query plans due to optimizer's cardinality estimation errors.
%We first invoke the optimizer to generate a plan as usual, and use sampling to refine cardinality estimates only for this single optimal plan.
%We then invoke the optimizer again by also feeding it the refined cardinality estimates to generate a perhaps different plan.
%This gives the optimizer second chance to generate a better plan if there were significant errors in the histogram-based cardinality estimates.
If there are significant errors, we use an iterative procedure to give the optimizer a chance to generate a better plan.
%We repeat this optimization-then-validation loop until the chosen plan is fixed.
%We further study this re-optimization procedure in detail, both theoretically and experimentally.
We study this re-optimization procedure in detail, both theoretically and experimentally.
Our theoretical analysis suggests that the efficiency of this procedure and the quality of the final plan returned can be guaranteed under certain assumptions, and our experimental evaluation on the TPC-H benchmark database as well as our own database with highly correlated data demonstrates the effectiveness of this approach.

\end{abstract} 

==> additional-experiments.tex <==
\section{Other Experimental Results} \label{appendix:sec:experiments}

%In this section, we report additional experimental results.

%\subsection{Results on TPC-H Database ($z=1$)} \label{appendix:sec:experiments:tpch-skew1}


%\subsection{Results on TPC-H Database ($z=2$)} \label{appendix:sec:experiments:tpch-skew2}
%
%Figure~\ref{fig:tpch-skew2:time} presents the running times of the queries over the more skewed TPC-H database, with or without calibration of the cost units.
%Figure~\ref{fig:tpch-skew2:num} and~\ref{fig:tpch-skew2:time-sampling} further present the number of plans considered during re-optimization and the running times excluding/including the re-optimization times.
%We can observe similar patterns as that over the databases with $z=0$ and $z=1$.
%
%\begin{figure}
%\centering
%\subfigure[Without calibration of the cost units]{ \label{fig:tpch-skew2:time:no-calib}
%\includegraphics[width=\columnwidth]{./figs/reopt-new-join-only-with-dev-skew2-time-no-calib.eps}}
%\subfigure[With calibration of the cost units]{ \label{fig:tpch-skew2:time:calib}
%\includegraphics[width=\columnwidth]{./figs/reopt-new-join-only-with-dev-skew2-time-calib.eps}}
%\caption{Query running time over skewed 10GB TPC-H database ($z=2$)}
%\label{fig:tpch-skew2:time}
%\shrink
%\end{figure}
%
%\begin{figure}
%\centering
%\includegraphics[width=\columnwidth]{./figs/reopt-new-join-only-with-dev-skew2-num.eps}
%\caption{The number of plans generated during re-optimization over skewed 10GB TPC-H database ($z=2$)}
%\label{fig:tpch-skew2:num}
%\shrink
%\end{figure}
%
%\begin{figure}
%\centering
%\subfigure[Without calibration of the cost units]{ \label{fig:tpch-skew2:time-sampling:no-calib}
%\includegraphics[width=\columnwidth]{./figs/reopt-new-join-only-with-dev-skew2-time-sampling-no-calib.eps}}
%\subfigure[With calibration of the cost units]{ \label{fig:tpch-skew2:time-sampling:calib}
%\includegraphics[width=\columnwidth]{./figs/reopt-new-join-only-with-dev-skew2-time-sampling-calib.eps}}
%\caption{Query running time excluding/including re-optimization time over skewed 10GB TPC-H database ($z=2$)}
%\label{fig:tpch-skew2:time-sampling}
%\shrink
%\end{figure}


%\subsection{Results of the Optimizer Torture Test} \label{appendix:sec:experiments:hdc}

Figure~\ref{fig:hdc:num} presents the number of plans generated during the re-optimization procedure for the 4-join and 5-join OTT queries.
Figure~\ref{fig:hdc-4:time-sampling} and~\ref{fig:hdc-5:time-sampling} further present the comparisons of the running times excluding/including re-optimization times for these queries (the $y$-axes are in log scale).

%Quite interestingly, we find that the number of plans generated coincides with the cases that re-optimization indeed identified the empty sub-queries: more plans were attempted during re-optimization.
%Meanwhile, the time spent on re-optimization remains trivial.

\begin{figure}
\centering
\subfigure[4-join queries]{ \label{fig:hdc:num:4-join}
\includegraphics[width=\columnwidth]{./figs/results-ext-reopt-new-join-only-4-num-no-self-joins.eps}}
\subfigure[5-join queries]{ \label{fig:hdc:num:5-join}
\includegraphics[width=\columnwidth]{./figs/results-ext-reopt-new-join-only-5-num-no-self-joins.eps}}
\caption{The number of plans generated during re-optimization for the OTT queries.}
\label{fig:hdc:num}
\shrink
\end{figure}

\begin{figure}%[!htb]
\centering
\subfigure[Without calibration of the cost units]{ \label{fig:hdc-4:time-sampling:no-calib}
\includegraphics[width=\columnwidth]{./figs/results-ext-reopt-new-join-only-4-time-sampling-no-calib-no-self-joins.eps}}
\subfigure[With calibration of the cost units]{ \label{fig:hdc-4:time-sampling:calib}
\includegraphics[width=\columnwidth]{./figs/results-ext-reopt-new-join-only-4-time-sampling-calib-no-self-joins.eps}}
\caption{Query running time excluding/including re-optimization time for the 4-join OTT queries.}
\label{fig:hdc-4:time-sampling}
\shrink
\end{figure}

\begin{figure}%[!hb]
\centering
\subfigure[Without calibration of the cost units]{ \label{fig:hdc-5:time-sampling:no-calib}
\includegraphics[width=\columnwidth]{./figs/results-ext-reopt-new-join-only-5-time-sampling-no-calib-no-self-joins.eps}}
\subfigure[With calibration of the cost units]{ \label{fig:hdc-5:time-sampling:calib}
\includegraphics[width=\columnwidth]{./figs/results-ext-reopt-new-join-only-5-time-sampling-calib-no-self-joins.eps}}
\caption{Query running time excluding/including re-optimization time for the 5-join OTT queries.}
\label{fig:hdc-5:time-sampling}
\shrink
\end{figure} 

Except for results over PostgreSQL, Figure~\ref{fig:db2:time} and~\ref{fig:sqlserver:time} present running times of the OTT queries over two commercial database systems. The results are similar to that over PostgreSQL. Again, the $y$-axes are in log scale and we do not show queries that finished in less than 0.1 second.

\begin{figure}%[!htb]
\centering
\subfigure[4-join OTT queries]{ \label{fig:db2:time:4-join}
\includegraphics[width=\columnwidth]{./figs/result-hdc-no-self-joins-DB2-4-join.eps}}
\subfigure[5-join OTT queries]{ \label{fig:db2:time:5-join}
\includegraphics[width=\columnwidth]{./figs/result-hdc-no-self-joins-DB2-5-join.eps}}
\caption{Query running times of the OTT queries on the commercial database system A.}
\label{fig:db2:time}
\shrink
\end{figure}

\begin{figure}%[!hb]
\centering
\subfigure[4-join OTT queries]{ \label{fig:sqlserver:time:4-join}
\includegraphics[width=\columnwidth]{./figs/result-hdc-no-self-joins-SQLServer-4-join.eps}}
\subfigure[5-join OTT queries]{ \label{fig:sqlserver:time:5-join}
\includegraphics[width=\columnwidth]{./figs/result-hdc-no-self-joins-SQLServer-5-join.eps}}
\caption{Query running times of the OTT queries on the commercial database system B.}
\label{fig:sqlserver:time}
\shrink
\end{figure}

==> algorithm.tex <==
\section{The Re-Optimization Algorithm}\label{sec:algorithm}

In this section, we first introduce necessary background information and terminology, and then present the details of the re-optimization algorithm. We focus on using sampling to refine selectivity estimates for join predicates. As was recently pointed out by Guy Lohman~\cite{Lohman-critique}, while histogram-based approaches have worked well for estimating selectivities of local predicates (i.e., predicates over a column of a single base table), accurate estimation of selectivities for join predicates (and how to combine them) remains challenging.
The sampling-based selectivity estimator we used is tailored for join queries~\cite{Haas-sample96}, and it is our goal in this paper to study its effectiveness in query optimization when combined with our proposed re-optimization procedure.
Nonetheless, sampling can also be used to estimate selectivities for other types of operators, such as aggregates (i.e., ``Group By'' clauses) that require estimation of the number of distinct values (e.g.~\cite{Charikar-sample00}). We leave the exploration of integrating other sampling-based selectivity estimation techniques into query optimization as interesting future work.

\subsection{Preliminaries}

In previous work~\cite{WuCHN13,WuCZTHN13,WuWHN14}, the authors used a sampling-based selectivity estimator proposed by Haas et al.~\cite{Haas-sample96} for the purpose of predicting query running times. In the following, we provide an informal description of this estimator.

Let $R_1$, ..., $R_K$ be $K$ relations, and let $R_k^s$ be the sample table of $R_k$ for $1\leq k\leq K$. Consider a join query $q=R_1\bowtie\cdots\bowtie R_K$. The selectivity $\rho_q$ of $q$ can be estimated as
$$\hat{\rho}_q = \frac{|R_1^s\bowtie\cdots\bowtie R_K^s|}{|R_1^s|\times\cdots\times|R_K^s|}.$$
It has been shown that this estimator is both unbiased and strongly consistent~\cite{Haas-sample96}: the larger the samples are, the more accurate this estimator is. Note that this estimator can be applied to joins that are sub-queries of $q$ as well.
%In~\cite{WuCZTHN13} we therefore presented a natural bottom-up procedure to estimate selectivities (and thus cardinalities) for all joins in a given query plan. We refer interested readers to~\cite{WuCZTHN13} for more details of this procedure.

\subsection{Algorithm Overview}

As mentioned in the introduction, cardinality estimation is challenging and cardinality estimates by optimizers can be erroneous.
This potential error can be noticed once we apply the aforementioned sampling-based estimator to the query plan generated by the optimizer.
%In our previous work, we stopped at this stage because our goal was to get a more accurate prediction of query running time rather than make the query run faster.
However, if there are really significant errors in cardinality estimates, the optimality of the plan returned by the optimizer can be in doubt.

%If we let the optimizer know the refined cardinality estimates obtained via sampling
If we replace the optimizer's cardinality estimates with sampling-based estimates and ask it to re-optimize the query, what would happen? Clearly, the optimizer will either return the same query plan, or a different one. In the former case, we can just go ahead to execute the query plan:
%the optimizer insists that the plan is optimal even if it knows there are errors in cardinality estimates.
the optimizer does not change plans even with the new cardinalities.
In the latter case, %the optimizer admits that the previous plan is not optimal.
the new cardinalities cause the optimizer to change plans.
However, this new plan may still not be trustworthy because the optimizer may still decide its optimality based on erroneous cardinality estimates. To see this, let us consider the following example.
\begin{example}\label{ex:joins-not-covered}
Consider the two join trees $T_1$ and $T_2$ in Figure~\ref{fig:transformations}.
Suppose that the optimizer first returns $T_1$ as the optimal plan.
Sampling-based validation can then refine cardinality estimates for the three joins: $A\bowtie B$, $A\bowtie B\bowtie C$, and $A\bowtie B\bowtie C\bowtie D$.
Upon knowing these refined estimates, the optimizer then returns $T_2$ as the optimal plan.
However, the join $C\bowtie D$ in $T_2$ is not observed in $T_1$ and its cardinality has not been validated.
\end{example}
Hence, we can again apply the sampling-based estimator to this new plan and repeat the re-optimization process. This then leads to an iterative procedure.

Algorithm~\ref{alg:reoptimization} outlines the above idea. Here, we use $\Gamma$ to represent the sampling-based cardinality estimates for joins that have been validated by using sampling. Initially, $\Gamma$ is empty. In the round $i$ ($i\geq 1$), the optimizer generates a query plan $P_i$ based on the current information preserved in $\Gamma$ (line 5). If $P_i$ is the same as $P_{i - 1}$, then we can terminate the iteration (lines 6 to 8). Otherwise, $P_i$ is new and we invoke the sampling-based estimator over it (line 9). We use $\Delta_i$ to represent the sampling-based cardinality estimates for $P_i$, and we update $\Gamma$ by merging $\Delta_i$ into it (line 10). We then move to the round $i + 1$ and repeat the above procedure (line 11).

%until $\Gamma$ does not change (line 11). As we will see in Section~\ref{sec:analysis}, the stability of $\Gamma$ guarantees the stability of the optimal plan returned by the optimizer.

\begin{algorithm}
  \SetAlgoLined
  \KwIn{$q$, a given SQL query}
  \KwOut{$P_q$, query plan of $q$ after re-optimization}
  \SetAlgoLined
  $\Gamma \leftarrow \emptyset$\;
  $P_0\leftarrow \Null$\;
  $i\leftarrow 1$\;
  \While {true} {
    $P_i\leftarrow GetPlanFromOptimizer(\Gamma)$\;
    \If{$P_i$ is the same as $P_{i-1}$} {
        \textbf{break}\;
    }
    $\Delta_i\leftarrow GetCardinalityEstimatesBySampling(P_i)$\;
    $\Gamma\leftarrow\Gamma\cup\Delta_i$\;
    $i\leftarrow i + 1$\;
  }
  Let the final plan be $P_q$\;
  \Return{$P_q$\;}
  \caption{Sampling-based query re-optimization}
\label{alg:reoptimization}
\end{algorithm}

In our current implementation of Algorithm~\ref{alg:reoptimization}, we implemented $\Gamma$ as a hash map where the keys are the joins and the values are the corresponding cardinalities.
When the optimizer needs to estimate the cardinality of a join, it first looks up $\Gamma$ to see if the join is present.
If yes, then it simply uses the recorded cardinality.
Otherwise, it invokes the histogram-based approaches to estimate the cardinality of the join as usual.

Note that this iterative process has as its goal improving the selected plan, not
finding a new globally optimal plan. It is certainly possible that the
iterative process misses a good plan because the iterative process
does not explore the complete plan space --- it only explores neighboring transformations of the chosen plan.
Nonetheless, as we will see in Section~\ref{sec:experiments}, this local search is sufficient to catch and
repair some very bad plans.

%We have two remarks regarding the implementation of Algorithm~\ref{alg:reoptimization}.
%First, $\Gamma$ can be simply implemented as a hash map where the keys are the joins and the values are the corresponding cardinalities.
%When the optimizer needs to estimate the cardinality of a join, it first looks up $\Gamma$ to see if the join is present.
%If yes, then it simply uses the recorded cardinality.
%Otherwise, it invokes the histogram-based approaches to estimate the cardinality of the join as usual.
%Second, note that the optimal plans returned by the optimizer may share joins (Example~\ref{ex:joins-not-covered}).
%A more efficient way might be to use sampling only for new joins that have not been seen so far.
%However, its implementation seems to be much more complicated so we leave it as future work.




==> analysis.tex <==

\begin{figure}
\centering
\includegraphics[width=0.9\columnwidth]{./figs/transformations.eps}
\caption{Join trees and their local transformations.}
\label{fig:transformations}
\shrink
\end{figure}

\section{Theoretical Analysis} \label{sec:analysis}

In this section, we present an analysis of Algorithm~\ref{alg:reoptimization} from a theoretical point of view. We are interested in two respects of the re-optimization procedure:
\begin{itemize}
\item \emph{Efficiency}, i.e., how many rounds of iteration does it require before it terminates?
\item \emph{Effectiveness}, i.e., how good is the final plan it returns compared to the original plan, in terms of the cost metric used by the query optimizer?
\end{itemize}
Our following study suggests that (i) the expected number of rounds of iteration in the worst case is upper-bounded by $O(\sqrt{N})$ where $N$ is the number of query plans explored in the optimizer's search space (Section~\ref{sec:analysis:efficiency}); and (ii) the final plan is guaranteed to be no worse than the original plan if
%the cost model satisfies some necessary conditions.
sampling-based cost estimates are consistent with the actual costs (Section~\ref{sec:analysis:optimality}).

\subsection{Notation and Definitions}

We start by introducing notation and establishing necessary definitions that will be used throughout our analysis.

\subsubsection{Structural Equivalence}

We use $\tree(P)$ to denote the join tree of a query plan $P$.

\begin{definition}[Structurally Equivalent Plans]
Two plans $P$ and $P'$ are \emph{structurally equivalent} if $\tree(P)$ and $\tree(P')$ are the same.
\end{definition}

In other words, structurally equivalent plans have the same join order of the relations; they only differ in the specific choices of physical operators (e.g., hash join vs. sort-merge join).

\subsubsection{Local and Global Transformations} \label{sec:analysis:transformations}

We further represent a join tree with a bottom-up, left-to-right encoding. Consider the following example.
\begin{example} [Encodings of Join Trees] \label{ex:join-tree-encoding}
Suppose we have a join query over four relations $A$, $B$, $C$, and $D$ with the join graph
$$G=\{(A, B), (C, D), (A, C), (A, D)\}.$$
In Figure~\ref{fig:transformations}, we present one left-deep tree plan $T_1$ and one bushy tree plan $T_2$ of the query.
The following are encodings of $T_1$ and $T_2$:
\begin{enumerate}[(T1)]
\item $((A\bowtie B)\bowtie C)\bowtie D \encoding (AB, ABC, ABCD)$;
\item $(A\bowtie B)\bowtie (C\bowtie D)\encoding (AB, CD, ABCD)$.
\end{enumerate}
\end{example}
We use $\code(T)$ to represent the encoding of a join tree $T$.

\begin{definition}[Local/Global Transformations]
Let $T$ and $T'$ be two join trees. $T'$ is a \emph{local} transformation of $T$ if the following conditions hold:
\begin{enumerate}[(1)]
\item $\forall J\in\code(T)$, there is $J'\in\code(T')$ such that $J'$ is a permutation of $J$;
\item $\code(T')$ is itself a permutation of $\code(T)$.
\end{enumerate}
Otherwise, $T'$ is a \emph{global} transformation of $T$.
\end{definition}

Intuitively, local transformations are subject to only exchanges of left and right subtrees.
For example, in Figure~\ref{fig:transformations} we further present two join trees $T'_1$ and $T'_2$ that are local transformations of $T_1$ and $T_2$, with the following encodings:
\begin{enumerate}[(T1')]
\item $(C\bowtie(A\bowtie B))\bowtie D \encoding (AB, CAB, CABD)$;
\item $(C\bowtie D)\bowtie (A\bowtie B) \encoding (CD, AB, CDAB)$.
\end{enumerate}

Given two plans $P$ and $P'$, we also say that $P'$ is a local/global transformation of $P$ if $\tree(P')$ is a local/global transformation of $\tree(P)$. Since by definition a join tree is a local transformation of itself, it then holds that
\begin{lemma}
If two plans $P$ and $P'$ are structurally equivalent, then $P'$ is a local transformation of $P$.
\end{lemma}

\subsection{Convergence Conditions}

At a first glance, even the convergence of Algorithm~\ref{alg:reoptimization} is questionable. Would it be possible that Algorithm~\ref{alg:reoptimization} keeps looping without termination? For instance, it seems to be possible that the re-optimization procedure might alternate between two plans $P1$ and $P2$, i.e., the plans generated by the optimizer are $P1$, $P2$, $P1$, $P2$, ...
As we will see, this is impossible and Algorithm~\ref{alg:reoptimization} is guaranteed to terminate. We next present a sufficient condition for the convergence of the re-optimization procedure. We first need one more definition regarding plan coverage.

\begin{definition}[Plan Coverage]\label{definition:plan-coverage}
Given a query plan $P$ and a set of query plans $\mathcal{P}$, $P$ is \emph{covered} by $\mathcal{P}$ if
$$\tree(P)\subseteq \bigcup\nolimits_{P'\in\mathcal{P}}\tree(P').$$
\end{definition}
That is, all the joins in the join tree of $P$ are included in the join trees of $\mathcal{P}$. As a special case, any plan that belongs to $\mathcal{P}$ is covered by $\mathcal{P}$.

Let $P_i$ ($i\geq 1$) be the plan returned by the optimizer in the $i$-th re-optimization step.

\begin{theorem}[Condition of Convergence]\label{theorem:convergence}
The re-optimization procedure terminates after $n + 1$ ($n\geq 1$) steps if $P_n$ is covered by $\mathcal{P}=\{P_1, ..., P_{n-1}\}$.
\end{theorem}

\begin{proof}
If $P_n$ is covered by $\mathcal{P}$, then using sampling-based validation would not contribute anything new to
the statistics $\Gamma$. That is, $\Delta_n\cup\Gamma = \Gamma$. Therefore, $P_{n+1}$ would be the same as $P_n$, because the optimizer would see the same $\Gamma$ in the round $n+1$ as that in the round $n$. Algorithm~\ref{alg:reoptimization} then terminates accordingly (by lines 6 to 8).
\end{proof}
%The proof is included in Appendix~\ref{appendix:sec:proofs:theorem:convergence}.
Note that the convergence condition stated in Theorem~\ref{theorem:convergence} is sufficient by not necessary. It could happen that $P_n$ is not covered by the previous plans $\{P_1,...,P_{n-1}\}$ but $P_{n+1}=P_n$ after using the validated statistics.

\begin{corollary}[Convergence Guarantee]\label{corollary:termination}
The re-optimization procedure is guaranteed to terminate.
\end{corollary}

\begin{proof}
Based on Theorem~\ref{theorem:convergence}, the re-optimization procedure would only continue if $P_n$ is not covered by $\mathcal{P}=\{P_1, ..., P_{n-1}\}$. In that case, $P_n$ should contain at least one join that has not been included by the plans in $\mathcal{P}$. Since the total number of possible joins considered by the optimizer is finite, $\mathcal{P}$ would eventually reach some fixed point if it kept growing. The re-optimization procedure is guaranteed to terminate upon that fixed point, again by Theorem~\ref{theorem:convergence}.
\end{proof}

%The proof is included in Appendix~\ref{appendix:sec:proofs:corollary:termination}.
Theorem~\ref{theorem:convergence} also implies the following special case:
\begin{corollary}\label{corollary:local-transformation}
The re-optimization procedure terminates after $n+1$ ($n\geq 1$) steps if $P_n\not\in\mathcal{P}$ but $P_n$ is a local transformation of some $P\in\mathcal{P}=\{P_1, ..., P_{n-1}\}$.
\end{corollary}

\begin{proof}
If $P_n$ is a local transformation of some $P\in\mathcal{P}$, then $\tree(P_n)$ and $\tree(P)$ contain the same joins. By Definition~\ref{definition:plan-coverage}, $P_n$ is covered by $\mathcal{P}$. Therefore, the re-optimization procedure terminates after $n+1$ steps, by Theorem~\ref{theorem:convergence}.
\end{proof}
Also note that Corollary~\ref{corollary:local-transformation} has covered the case that $P_n$ is a local transformation of (or even structurally equivalent to) $P_{n-1}$, which is very common in practice.

Based on Corollary~\ref{corollary:local-transformation}, we next present an important property of the re-optimization procedure.
\begin{theorem}\label{theorem:sequence-transformation}
When the re-optimization procedure terminates, exactly one of the following three cases could happen:
\begin{enumerate}[(1)]
\item It terminates after 2 steps with $P_2=P_1$.
\item It terminates after $n+1$ steps ($n > 1$). For $1\leq i\leq n$, $P_i$ is a global transformation of $P_j$ with $j < i$.
\item It terminates after $n+1$ steps ($n > 1$). For $1\leq i\leq n - 1$, $P_i$ is a global transformation of $P_j$ with $j < i$, and $P_n$ is a local transformation of some $P\in\mathcal{P}=\{P_1,...,P_{n-1}\}$.
\end{enumerate}
\end{theorem}
That is, when the procedure does not terminate trivially (Case (1)), it could be characterized as a sequence of global transformations with \emph{at most} one more local transformation before its termination (Case (2) or (3)). Figure~\ref{fig:sequence-of-transformations} illustrates the latter two nontrivial cases. A formal proof of Theorem~\ref{theorem:sequence-transformation} is included in Appendix~\ref{appendix:sec:proofs:theorem:sequence-transformation}.

\begin{figure}
\centering
\includegraphics[width=0.9\columnwidth]{./figs/sequence-of-transformations.eps}
\caption{Characterization of the re-optimization procedure ($g$ and $l$ stand for global and local transformations, respectively). For ease of illustration, $P_i$ is only noted as a global transformation of $P_{i-1}$, but we should keep in mind that $P_i$ is also a global transformation of all the $P_j$'s with $j < i$.}
\label{fig:sequence-of-transformations}
\shrink
\end{figure}

\subsection{Efficiency}\label{sec:analysis:efficiency}

We are interested in how fast the re-optimization procedure can terminate. As pointed out by Theorem~\ref{theorem:sequence-transformation}, the convergence speed depends on the number of \emph{global} transformations the procedure undergoes. In the following, we first develop a probabilistic model that will be used in our analysis, and then present analytic models for the general case and several important special cases.

\subsubsection{A Probabilistic Model}

Consider a queue of $N$ balls. Originally all balls are not marked. We then conduct the following procedure:

\begin{procedure}\label{procedure:random-ball-model}
In each step, we pick the ball at the head of the queue. If it is marked, then the procedure terminates. Otherwise, we mark it and randomly insert it back into the queue. The probability that the ball would be inserted at the position $i$ ($1\leq i \leq N$) is uniformly $1/N$.
\end{procedure}

We next study the expected number of steps that Procedure~\ref{procedure:random-ball-model} would take before its termination.

\begin{lemma}\label{lemma:expected-steps}
The expected number of steps that Procedure~\ref{procedure:random-ball-model} would take before its termination is:
\begin{equation}\label{eq:SN}
S_N=\sum_{k=1}^N k\cdot(1-\frac{1}{N})\cdots(1-\frac{k-1}{N})\cdot\frac{k}{N}.
\end{equation}
\end{lemma}

The proof of Lemma~\ref{lemma:expected-steps} is in Appendix~\ref{appendix:sec:proofs:lemma:expected-steps}.
While a closed form of $S_N$ in Equation~\ref{eq:SN} does not exist, we can show that $S_N$ is bounded by $O(\sqrt{N})$.

\begin{theorem}\label{theorem:SN-upper-bound}
The expected number of steps $S_N$ as presented in Lemma~\ref{lemma:expected-steps} satisfies $S_N = O(\sqrt{N})$.
\end{theorem}

The proof of Theorem~\ref{theorem:SN-upper-bound} is in Appendix~\ref{appendix:sec:proofs:theorem:SN-upper-bound}.
In Figure~\ref{fig:sN}, we plot $S_N$ by increasing $N$ from $1$ to $1000$.
As we can see, the growth speed of $S_N$ is very close to that of $f(N)=\sqrt{N}$.

\begin{figure}
\centering
\includegraphics[width=\columnwidth]{./figs/s_N.eps}
\caption{$S_N$ with respect to the growth of $N$.}
\label{fig:sN}
\shrink
\end{figure}

%Table~\ref{tab:SN} lists the $S_N$ with respect to the growth of $N$.
%
%\begin{table}[th]
%\small
%\centering
%\begin{tabular}{|l|r|r|r|r|r|r|r|r|r|r|}
%  \hline
%$N$& 1 & 10 & 20 & 30 & 40 & 50 & 60 & 70 & 80 & 90\\
%$S_N$ & 1 & 3 & 5 & 6 & 7 & 8 & 9 & 10 & 10 & 11\\
%  \hline \hline
%$N$ & 100 & 200 & 300 & 400 & 500 & 600 & 700 & 800 & 900 & 1000\\
%$S_N$ & 12 & 17 & 21 & 24 & 27 & 30 & 32 & 35 & 37 & 39\\
%  \hline
%\end{tabular}
%\caption{$S_N$ with respect to the growth of $N$}
%\label{tab:SN}
%\shrink
%\end{table}

\subsubsection{The General Case}

In a nutshell, query optimization could be thought of as picking a plan with the lowest estimated cost among a number of candidates. Different query optimizers have different search spaces, so in general we can only assume a search space with $N$ different join trees that would be considered by an optimizer.\footnote{By ``different'' join trees, we mean join trees that are global transformations of each other. We use this convention in the rest of the paper unless specific clarifications are noted.} Let these trees be $T_1$, ..., $T_N$, ordered by their estimated costs. The re-optimization procedure could then be thought of as shuffling these trees based on their refined cost estimates. This procedure terminates whenever (or even before) the tree with lowest estimated cost reoccurs, that is, when some tree appears at the head position for the second time. Therefore, the probabilistic model in the previous section applies here. As a result, by Lemma~\ref{lemma:expected-steps}, the expected number of steps for this procedure to terminate is $S_N$. We formalize this result as the following theorem:

\begin{theorem} \label{theorem:efficiency}
Assume that the position of a plan (after sampling-based validation) in the ordered plans with respect to their costs is uniformly distributed.
Let $N$ be the number of different join trees in the search space.
The expected number of steps before the re-optimization procedure terminates is then $S_N$, where $S_N$ is computed by Equation~\ref{eq:SN}.
Moreover, $S_N=O(\sqrt{N})$ by Theorem~\ref{theorem:SN-upper-bound}.
\end{theorem}

We emphasize that the analysis here only targets worst-case performance, which might be too pessimistic. In our experiments, we have found that all queries we tested require less than 10 rounds of iteration, most of which require only 1 or 2 rounds.

\blankline

\remark{The uniformity assumption in Theorem~\ref{theorem:efficiency} may not be valid in practice. It is possible that a plan after sampling-based validation (or, a marked ball in terms of Procedure~\ref{procedure:random-ball-model}) is more likely to be inserted into the front/back half of the queue. Such cases imply that, rather than with an equal chance of overestimation/underestimation, the optimizer tends to overestimates/underestimates the costs of all query plans (for a particular query). This is, however, not impossible.
In practice, significant cardinality estimation errors usually appear locally and propagate upwards. Once the error at some join were corrected, the errors in all plans that contain that join would also be corrected. In other words, the correction of the error at a single join can lead to the correction of errors in many candidate plans. In Appendix~\ref{appendix:sec:analysis}, we further present analysis for two extreme cases: all local errors are overestimates/underestimates. Any real case sits in between.
To summarize, for left-deep join trees, we have the following two results:
\begin{itemize}
\item If all local errors are overestimates, then in the worst case the re-optimization procedure would terminate in at most $m+1$ steps, where $m$ is the number of joins in the query.
\item If all local errors are underestimates, then in the worst case the re-optimization procedure is expected to terminate in $S_{N/M}$ steps, where $N$ is the number of different join trees in the optimizer's search space and $M$ is the number of edges in the join graph.
\end{itemize}
Note that both results are better than the bound stated in Theorem~\ref{theorem:efficiency}.
For instance, in the underestimation-only case, if $N=1000$ and $M=10$, we have $S_N=39$ but $S_{N/M}=12$.}

%\todo{We can challenge the assumption used in the probabilistic model by saying that the ball is more likely to be inserted at the front/back half of the queue. In general, we can assume an arbitrary distribution of the likelihoods that a ball could be inserted back into the positions of the queue. Then we can do a simulation (e.g., Monte Carlo experiments) to compute the number of steps before the procedure terminates.}


%\paragraph{Overestimates And Underestimates}
%
%It is more natural in practice that both overestimates and underestimates could occur. The expected number of steps before the re-optimization procedure terminates is then between that of the two extreme cases discussed above.

\subsection{Optimality of the Final Plan} \label{sec:analysis:optimality}

We can think of the re-optimization procedure as progressive adjustments of the optimizer's direction when it explores its search space. Of course, the search space depends on the algorithm or strategy used by the optimizer, and thus the impact of re-optimization also depends on that.
But we can still have some general conclusions about the optimality of the final plan regardless of the search space.

\begin{assumption}\label{assumption:cost-function}
The cost estimates of plans after using sampling-based selectivity refinement are consistent. That is, for any two plans $P_1$ and $P_2$, if $\cost^s(P_1) < \cost^s(P_2)$, then $\cost^a(P_1) < \cost^a(P_2)$. Here, $\cost^s(P)$ and $\cost^a(P)$ are the estimated cost based on sampling and the actual cost of plan $P$.
\end{assumption}

We have the following theorem based on Assumption~\ref{assumption:cost-function}. The proof is included in Appendix~\ref{appendix:sec:proofs:theorem:local-optimality}.

\begin{theorem}\label{theorem:local-optimality}
Let $P_1$, ..., $P_n$ be a series of plans generated during re-optimization. Then $\cost^s(P_n)\leq \cost^s(P_i)$, and thus $\cost^a(P_n)\leq\cost^a(P_i)$ under Assumption~\ref{assumption:cost-function}, for $1\leq i \leq n - 1$.
\end{theorem}

That is, the plan after re-optimization is guaranteed to be better than the original plan. Nonetheless, it is difficult to conclude that the plans are improved monotonically, namely, in general it is not true that $\cost^s(P_{i+1})\leq\cost^s(P_i)$, for $1\leq i\leq n - 1$. However, we can prove that this is true if we only have overestimates (proof in Appendix~\ref{appendix:sec:proofs:corollary:local-optimality:overestimates}).

\begin{corollary} \label{corollary:local-optimality:overestimates}
If in re-optimization only overestimates occur, then $\cost^s(P_{i+1})\leq\cost^s(P_i)$ for $0\leq i\leq n$.
\end{corollary}

Our last result on the optimality of the final plan is in the sense that it is the best among all the plans that are local transformations of the final plan (proof in Appendix~\ref{appendix:sec:proofs:theorem:optimality-local-transformation}).

\begin{theorem}\label{theorem:optimality-local-transformation}
Let $P$ be the final plan returned by the re-optimization procedure. For any $P'$ such that $P'$ is a local transformation of $P$, it holds that $\cost^s(P)\leq\cost^s(P')$.
\end{theorem}
Again note that this implies that the final plan is the best among all the plans that have the same join tree.

\subsection{Discussion}

We call the final plan returned by the re-optimization procedure the \emph{fixed point} with respect to the initial plan generated by the optimizer. According to Theorem~\ref{theorem:local-optimality}, this plan is a \emph{local optimum} with respect to the initial plan. Note that, if $\mathcal{P} = \{P_1, ..., P_n\}$ covers the whole search space, that is, any plan $P$ in the search space is covered by $\mathcal{P}$, then the locally optimal plan obtained is also globally optimal.

A natural question is then the impact of the initial plan. Intuitively, it seems that the initial plan can affect both the fixed point and the time it takes to converge to the fixed point. (Note that it is straightforward to prove that the fixed point must exist and be unique, with respect to the given initial plan.) There are also other related interesting questions. For example, if we start with two initial plans with similar cost estimates, would they converge to fixed points with similar costs as well? We leave all these problems as interesting directions for further investigation.

Moreover, the convergence of the re-optimization procedure towards a fixed point can also be viewed as a validation procedure of the costs of the plans $\mathcal{V}$ that can be covered by $\mathcal{P}=\{P_1, ..., P_n\}$. Note that $\mathcal{V}$ is a subset of the whole search space explored by the optimizer, and $\mathcal{V}$ is induced by $P_1$ --- the initial plan that is deemed as optimal by the optimizer. It is also interesting future work to study the relationship between $P_1$ and $\mathcal{V}$, especially how much of the complete search space can be covered by $\mathcal{V}$.


%\begin{algorithm}
%  \SetAlgoLined
%  \KwIn{$q$, a given SQL query}
%  \KwOut{$P_q$, query plan of $q$ after re-optimization}
%  \SetAlgoLined
%  $\Gamma \leftarrow \emptyset$\;
%  $P_0\leftarrow \Null$\;
%  $i\leftarrow 1$\;
%  \Repeat {no\ new\ statistics\ added\ to\ $\Gamma$} {
%    $P_i\leftarrow GetPlanFromOptimizer(\Gamma)$\;
%    \If{$P_i$ is the same as $P_{i-1}$} {
%        \textbf{break}\;
%    }
%    $\Delta_i\leftarrow GetCardinalityEstimatesBySampling(P_i)$\;
%    \If{$\cost(P_i)^{\sampling}\geq \cost(P_i)^{\optimizer}$} {
%        \textbf{break}\;
%    }
%
%    $\Gamma\leftarrow\Gamma\cup\Delta_i$\;
%    $i\leftarrow i + 1$\;
%  }
%  Let the final plan be $P_q$\;
%  \Return{$P_q$\;}
%  \caption{Sampling-based query re-optimization (conservative version)}
%\label{alg:reoptimization-conservative}
%\end{algorithm} 

==> analysisBackup.tex <==
\paragraph{Underestimates Only}

Suppose that, on the other hand, the error is an underestimate, that is, the actual cardinality is larger than the one estimated by the optimizer. Then rather than just those plans with the erroneous node as subtrees, the one with the lowest estimated cost in the rest of the search space also has the potential of being the optimal one after correcting the estimation error. We want to know the probability that a new plan would come from the former and that of the latter.

Formally, let the search space contain $N$ join trees in total, and let $N_1$ be the number of join trees in the former case. The probability that a new plan $P'$ would belong to the latter case is ratio between the number of permutations of the $N$ join trees such that $P'$ is the head and the number of all permutations.

The number of all such permutations is $\frac{N!}{(N-N_1)!}$, and the number of permutations that $P'$ is the first is $\frac{(N-1)!}{(N-N_1-1)!}$. As a result, the desired probability is $\frac{N-N_1}{N}=1-\frac{N_1}{N}$. So the probability that a new plan will remain in the former category is $1-(1-\frac{N_1}{N})=\frac{N_1}{N}$.

If each time the new plan remains in the former category even if the errors are underestimates, then following Theorem~\ref{theorem:overestimate} we know that the procedure would terminate in at most $m+2$ steps. Otherwise we would have a new plan in the latter category, which means that the plan will have no overlap with the current one.

But, as we move on, it is less and less likely that we would come up with a new plan that is ``completely new'' in the sense that it has no overlap with all previously generated plans. Since we focus on left-deep trees, such a plan must have a different starting point, i.e., the first join in the plan is different from that of all previous plans. Suppose that the join graph contains $M$ edges and we have already observed $k$ of them. The probability that we would have a ``completely new'' plan is then $\frac{M-k}{M}=1-\frac{k}{M}$. In other words, with probability $\frac{k}{m}$ we would see a plan $P$ overlapping with some previous plan $P'$.

Our next concern is the probability that $P'$ would overlap with $P$ by $i$ joins, for $1\leq i\leq m$, where $m$ is the number of joins in the query.

Just another model for the case of underestimates and left-deep trees. Suppose that the join graph $G$ contains $M$ edges. We partition the join trees based on their first joins, which must be the edges of $G$. So we have $M$ partitions in total.

Let $s_i$ be the state when a plan returned by the optimizer with its first join the $i$-th edge in $G$ ($1\leq i\leq M$). The re-optimization procedure could then be though of as transitions between these $M$ states, i.e., a Markov chain. As before, we assume that the transition probabilities are uniform, i.e., $\pi(s_j|s_i)=\frac{1}{M}$ for $1\leq i,j\leq M$. In other words, it is equally likely that the next plan generated would have its first join in the partition $i$ for $1\leq i\leq M$. Then the equilibrium state distribution of this Markov chain is also uniform. That is, given any plan generated in the re-optimization procedure, it is equally likely that it would have its first join in the partition $i$ for $1\leq i\leq M$. We could estimate the expected number of steps before the procedure terminates as $S=\sum_{i=1}^M \pi(s_i)\cdot N_i$, where $N_i$ is the number of steps/transitions confined in the partition $i$ before termination. Since we only consider left-deep trees, $N_i=N_j$ for $1\leq i,j\leq M$. As a result, $S$ could be simplified as $S=N_i$. So we are left with estimating $N_i$.

$N_i$ is the expected number of steps before termination if the transitions (i.e., re-optimization steps) are confined in the partition $i$. We could divide this process into stages, while each stage contains one more join than the previous stage, just like one stage in the classic dynamic programming procedure. If there are $m$ joins, then we would have $m$ stages. In each stage, we go through every plan until we finish, and the average number of plans we considered is $S_{K_j}$ as computed by Equation~\ref{eq:SN}, where $K_j$ is the number of join-trees (actually subtrees) in the stage $j$ ($1\leq j\leq m$). So $S=N_i=\sum_{j=1}^m S_{K_j}$.
As an upper bound, we have $S\leq S_{N/M}$, where $N$ is the total number of join trees considered by the optimizer, and $S_{N/M}$ is computed according to Equation~\ref{eq:SN}. Note that $S_{N/M}$ is usually much smaller than $S_N$, according to Table~\ref{tab:SN}.

\paragraph{Overestimates And Underestimates}

It is more natural in practice that both overestimates and underestimates could occur. The expected number of steps before the re-optimization procedure terminates is then between that of the two extreme cases discussed above.

\subsection{Optimality of the Final Plan}

We can think of the re-optimization procedure as adjusting the optimizer's direction when it explores its search space. Of course, the search space depends on the algorithm or strategy used by the optimizer, and thus the impact of re-optimization also depends on that.
But we can still have some general conclusions about the optimality of the final regardless of the search space.

\begin{assumption}\label{assumption:cost-function}
The cost estimates of plans after using sampling-based selectivity refinement are consistent. That is, for any two plans $P_1$ and $P_2$, if $\cost^e(P_1) < \cost^e(P_2)$, then $\cost^a(P_1) < \cost^a(P_2)$. Here, $\cost^e(P)$ and $\cost^a(P)$ are the estimated and actual costs of a plan $P$.
\end{assumption}

We have the following theorem based on Assumption~\ref{assumption:cost-function}.

\begin{theorem}\label{theorem:local-optimality}
Let $P_1$, ..., $P_n$ be a series of plans generated during re-optimization. Then $\cost(P_i)\geq\cost(P_n)$ for $1\leq i \leq n - 1$.
\end{theorem}

\begin{proof}
\end{proof}

That is, the plan after re-optimization is guaranteed to be better than the original plan. Nonetheless, it is difficult to conclude that the plans are improved monotonically, namely, in general it is not true that $\cost(P_i)\geq\cost(P_{i + 1})$, for $1\leq i\leq n - 1$. However, we can prove that this is true if we only have overestimates.

\begin{corollary}
If only overestimates occur in the re-optimization procedure, then $\cost(P_{i+1})\leq\cost(P_i)$ for $0\leq i\leq n$.
\end{corollary}

\begin{proof}
\end{proof}

\todo{We can prove the optimality of the plan in the sense that it is the best among all the plans that have the same join tree.}

\subsection{Discussion}

We call the final plan returned after the re-optimization procedure terminates the \emph{fixed point} with respect to the initial plan generated by the optimizer. According to Theorem~\ref{theorem:local-optimality}, this plan is a \emph{local optimality} with respect to the initial plan. Note that, if $\mathcal{P} = \{P_1, ..., P_n\}$ covers the whole search space, that is, any plan $P$ in the search space is covered by $\mathcal{P}$, then the locally optimal plan obtained is also globally optimal.

A natural question is then the impact of the initial plan. Intuitively, it seems that the initial plan can affect both the fixed point and the time it takes to converge to the fixed point. (Note that it is straightforward to prove that the fixed point must exist and be unique, with respect to the given initial plan.) There are also other related interesting questions. For example, if we start with two initial plans with similar cost estimates, would they converge to fixed points with similar costs as well?

The convergence towards a fixed point is actually a validation of the costs of the plans $\mathcal{P}$ that can be covered by $\{P_1, ..., P_n\}$ and finally the best one (i.e., the fixed point $P_n$) is determined as the optimal one. Note that $\mathcal{P}$ is induced by $P_1$, namely, the initial plan that is deemed as optimal by the optimizer. It is very interesting future work to study the relationship between $P_1$ and $\mathcal{P}$.


\begin{algorithm}
  \SetAlgoLined
  \KwIn{$q$, a given SQL query}
  \KwOut{$P_q$, query plan of $q$ after re-optimization}
  \SetAlgoLined
  $\Gamma \leftarrow \emptyset$\;
  $P_0\leftarrow \Null$\;
  $i\leftarrow 1$\;
  \Repeat {no\ new\ statistics\ added\ to\ $\Gamma$} {
    $P_i\leftarrow GetPlanFromOptimizer(\Gamma)$\;
    \If{$P_i$ is the same as $P_{i-1}$} {
        \textbf{break}\;
    }
    $\Delta_i\leftarrow GetCardinalityEstimatesBySampling(P_i)$\;
    \If{$\cost(P_i)^{\sampling}\geq \cost(P_i)^{\optimizer}$} {
        \textbf{break}\;
    }

    $\Gamma\leftarrow\Gamma\cup\Delta_i$\;
    $i\leftarrow i + 1$\;
  }
  Let the final plan be $P_q$\;
  \Return{$P_q$\;}
  \caption{Sampling-based query re-optimization (conservative version)}
\label{alg:reoptimization-conservative}
\end{algorithm} 

==> analysisNew-old.tex <==

\begin{figure}
\centering
\includegraphics[width=0.9\columnwidth]{./figs/transformations.eps}
\caption{Join trees and their local transformations.}
\label{fig:transformations}
\shrink
\end{figure}

\section{Theoretical Analysis} \label{sec:analysis}

In this section, we present an analysis of Algorithm~\ref{alg:reoptimization} from a theoretical point of view. We are interested in two respects of the re-optimization procedure:
\begin{itemize}
\item \emph{Efficiency}, i.e., how many rounds of iteration does it require before it terminates?
\item \emph{Effectiveness}, i.e., how good is the final plan it returns compared to the original plan, in terms of the cost metric used by the query optimizer?
\end{itemize}
Our following study suggests that (i) the expected number of rounds of iteration in the worst case is upper-bounded by $O(\sqrt{N})$ where $N$ is the number of query plans explored in the optimizer's search space (Section~\ref{sec:analysis:efficiency}); and (ii) the final plan is guaranteed to be no worse than the original plan if
%the cost model satisfies some necessary conditions.
sampling-based cost estimates are consistent with the actual costs (Section~\ref{sec:analysis:optimality}).

\subsection{Local and Global Transformations}

We start by introducing the notion of local/global transformations of query plans.
In the following, we use $\tree(P)$ to denote the join tree of a query plan $P$, which is represented as the \emph{set} of (logical) joins contained in $P$. For example, the representation of $T_1$ in Figure~\ref{fig:transformations} is $T_1=\{A\bowtie B, A\bowtie B\bowtie C, A\bowtie B\bowtie C\bowtie D\}$.

\begin{definition}[Local/Global Transformations]
Two join trees $T$ and $T'$ are \emph{local} transformations of each other if $T=T'$. Otherwise, they are global transformations.
\end{definition}

Intuitively, local transformations are subject to only exchanges of left/right subtrees and specific choices of physical join operators (e.g., hash join vs. sort-merge join).
For example, in Figure~\ref{fig:transformations} we further present two join trees $T'_1$ and $T'_2$ that are local transformations of $T_1$ and $T_2$.

Given two plans $P$ and $P'$, we also say that $P'$ is a local/global transformation of $P$ if $\tree(P')$ is a local/global transformation of $\tree(P)$.

\subsection{Convergence Conditions}

At a first glance, even the convergence of Algorithm~\ref{alg:reoptimization} is questionable. Would it be possible that Algorithm~\ref{alg:reoptimization} keeps looping without termination? For instance, it seems to be possible that the re-optimization procedure might alternate between two plans $P1$ and $P2$, i.e., the plans generated by the optimizer are $P1$, $P2$, $P1$, $P2$, ...
As we will see, this is impossible and Algorithm~\ref{alg:reoptimization} is guaranteed to terminate. We next present a sufficient condition for the convergence of the re-optimization procedure. We first need one more definition regarding plan coverage.

\begin{definition}[Plan Coverage]\label{definition:plan-coverage}
Given a query plan $P$ and a set of query plans $\mathcal{P}$, $P$ is \emph{covered} by $\mathcal{P}$ if
$$\tree(P)\subseteq \bigcup\nolimits_{P'\in\mathcal{P}}\tree(P').$$
\end{definition}
That is, all the joins in the join tree of $P$ are included in the join trees of $\mathcal{P}$. As a special case, any plan that belongs to $\mathcal{P}$ is covered by $\mathcal{P}$.

Let $P_i$ ($i\geq 1$) be the plan returned by the optimizer in the $i$-th re-optimization step.

\begin{theorem}[Condition of Convergence]\label{theorem:convergence}
The re-optimization procedure terminates after $n + 1$ ($n\geq 1$) steps if $P_n$ is covered by $\mathcal{P}=\{P_1, ..., P_{n-1}\}$.
\end{theorem}

\begin{proof}
If $P_n$ is covered by $\mathcal{P}$, then using sampling-based validation would not contribute anything new to
the statistics $\Gamma$. That is, $\Delta_n\cup\Gamma = \Gamma$. Therefore, $P_{n+1}$ would be the same as $P_n$, because the optimizer would see the same $\Gamma$ in the round $n+1$ as that in the round $n$. Algorithm~\ref{alg:reoptimization} then terminates accordingly (by lines 6 to 8).
\end{proof}
%The proof is included in Appendix~\ref{appendix:sec:proofs:theorem:convergence}.
Note that the convergence condition stated in Theorem~\ref{theorem:convergence} is sufficient by not necessary. It could happen that $P_n$ is not covered by the previous plans $\{P_1,...,P_{n-1}\}$ but $P_{n+1}=P_n$ after using the validated statistics (e.g., if there were no significant errors detected in cardinality estimates of $P_n$).

\begin{corollary}[Convergence Guarantee]\label{corollary:termination}
The re-optimization procedure is guaranteed to terminate.
\end{corollary}

\begin{proof}
Based on Theorem~\ref{theorem:convergence}, the re-optimization procedure would only continue if $P_n$ is not covered by $\mathcal{P}=\{P_1, ..., P_{n-1}\}$. In that case, $P_n$ should contain at least one join that has not been included by the plans in $\mathcal{P}$. Since the total number of possible joins considered by the optimizer is finite, $\mathcal{P}$ would eventually reach some fixed point if it kept growing. The re-optimization procedure is guaranteed to terminate upon that fixed point, again by Theorem~\ref{theorem:convergence}.
\end{proof}

%The proof is included in Appendix~\ref{appendix:sec:proofs:corollary:termination}.
Theorem~\ref{theorem:convergence} also implies the following special case:
\begin{corollary}\label{corollary:local-transformation}
The re-optimization procedure terminates after $n+1$ ($n\geq 1$) steps if $P_n\not\in\mathcal{P}$ but $P_n$ is a local transformation of some $P\in\mathcal{P}=\{P_1, ..., P_{n-1}\}$.
\end{corollary}

\begin{proof}
If $P_n$ is a local transformation of some $P\in\mathcal{P}$, then $\tree(P_n)$ and $\tree(P)$ contain the same joins. By Definition~\ref{definition:plan-coverage}, $P_n$ is covered by $\mathcal{P}$. Therefore, the re-optimization procedure terminates after $n+1$ steps, by Theorem~\ref{theorem:convergence}.
\end{proof}
Also note that Corollary~\ref{corollary:local-transformation} has covered a common case in practice that $P_n$ is a local transformation of $P_{n-1}$.

Based on Corollary~\ref{corollary:local-transformation}, we next present an important property of the re-optimization procedure.
\begin{theorem}\label{theorem:sequence-transformation}
When the re-optimization procedure terminates, exactly one of the following three cases could happen:
\begin{enumerate}[(1)]
\item It terminates after 2 steps with $P_2=P_1$.
\item It terminates after $n+1$ steps ($n > 1$). For $1\leq i\leq n$, $P_i$ is a global transformation of $P_j$ with $j < i$.
\item It terminates after $n+1$ steps ($n > 1$). For $1\leq i\leq n - 1$, $P_i$ is a global transformation of $P_j$ with $j < i$, and $P_n$ is a local transformation of some $P\in\mathcal{P}=\{P_1,...,P_{n-1}\}$.
\end{enumerate}
\end{theorem}
That is, when the procedure does not terminate trivially (Case (1)), it could be characterized as a sequence of global transformations with \emph{at most} one more local transformation before its termination (Case (2) or (3)). Figure~\ref{fig:sequence-of-transformations} illustrates the latter two nontrivial cases. A formal proof of Theorem~\ref{theorem:sequence-transformation} is included in Appendix~\ref{appendix:sec:proofs:theorem:sequence-transformation}.

\begin{figure}
\centering
\includegraphics[width=0.9\columnwidth]{./figs/sequence-of-transformations.eps}
\caption{Characterization of the re-optimization procedure ($g$ and $l$ stand for global and local transformations, respectively). For ease of illustration, $P_i$ is only noted as a global transformation of $P_{i-1}$, but we should keep in mind that $P_i$ is also a global transformation of all the $P_j$'s with $j < i$.}
\label{fig:sequence-of-transformations}
\shrink
\end{figure}

\subsection{Efficiency}\label{sec:analysis:efficiency}

We are interested in how fast the re-optimization procedure can terminate. As pointed out by Theorem~\ref{theorem:sequence-transformation}, the convergence speed depends on the number of \emph{global} transformations the procedure undergoes. In the following, we first develop a probabilistic model that will be used in our analysis, and then present analytic results for the general case and several important special cases.

\subsubsection{A Probabilistic Model}

Consider a queue of $N$ balls. Originally all balls are not marked. We then conduct the following procedure:

\begin{procedure}\label{procedure:random-ball-model}
In each step, we pick the ball at the head of the queue. If it is marked, then the procedure terminates. Otherwise, we mark it and randomly insert it back into the queue. The probability that the ball would be inserted at the position $i$ ($1\leq i \leq N$) is uniformly $1/N$.
\end{procedure}

We next study the expected number of steps that Procedure~\ref{procedure:random-ball-model} would take before its termination.

\begin{lemma}\label{lemma:expected-steps}
The expected number of steps that Procedure~\ref{procedure:random-ball-model} would take before its termination is:
\begin{equation}\label{eq:SN}
S_N=\sum_{k=1}^N k\cdot(1-\frac{1}{N})\cdots(1-\frac{k-1}{N})\cdot\frac{k}{N}.
\end{equation}
\end{lemma}

The proof of Lemma~\ref{lemma:expected-steps} is in Appendix~\ref{appendix:sec:proofs:lemma:expected-steps}.
While a closed form of $S_N$ in Equation~\ref{eq:SN} does not exist, we can show that $S_N$ is bounded by $O(\sqrt{N})$.

\begin{theorem}\label{theorem:SN-upper-bound}
The expected number of steps $S_N$ as presented in Lemma~\ref{lemma:expected-steps} satisfies $S_N = O(\sqrt{N})$.
\end{theorem}

The proof of Theorem~\ref{theorem:SN-upper-bound} is in Appendix~\ref{appendix:sec:proofs:theorem:SN-upper-bound}.
In Figure~\ref{fig:sN}, we plot $S_N$ by increasing $N$ from $1$ to $1000$.
As we can see, the growth speed of $S_N$ is very close to that of $f(N)=\sqrt{N}$.

\begin{figure}
\centering
\includegraphics[width=\columnwidth]{./figs/s_N.eps}
\caption{$S_N$ with respect to the growth of $N$.}
\label{fig:sN}
\shrink
\end{figure}

%Table~\ref{tab:SN} lists the $S_N$ with respect to the growth of $N$.
%
%\begin{table}[th]
%\small
%\centering
%\begin{tabular}{|l|r|r|r|r|r|r|r|r|r|r|}
%  \hline
%$N$& 1 & 10 & 20 & 30 & 40 & 50 & 60 & 70 & 80 & 90\\
%$S_N$ & 1 & 3 & 5 & 6 & 7 & 8 & 9 & 10 & 10 & 11\\
%  \hline \hline
%$N$ & 100 & 200 & 300 & 400 & 500 & 600 & 700 & 800 & 900 & 1000\\
%$S_N$ & 12 & 17 & 21 & 24 & 27 & 30 & 32 & 35 & 37 & 39\\
%  \hline
%\end{tabular}
%\caption{$S_N$ with respect to the growth of $N$}
%\label{tab:SN}
%\shrink
%\end{table}

\subsubsection{The General Case}

In a nutshell, query optimization can be thought of as picking a plan with the lowest estimated cost among a number of candidates. Different query optimizers have different search spaces, so in general we can only assume a search space with $N$ different join trees that would be considered by an optimizer.\footnote{By ``different'' join trees, we mean join trees that are global transformations of each other. We use this convention in the rest of the paper unless specific clarifications are noted.} Let these trees be $T_1$, ..., $T_N$, ordered by their estimated costs. The re-optimization procedure can then be thought of as shuffling these trees based on their refined cost estimates. This procedure terminates whenever (or even before) the tree with lowest estimated cost reoccurs, that is, when some tree appears at the head position for the second time. Therefore, the probabilistic model in the previous section applies here. As a result, by Lemma~\ref{lemma:expected-steps}, the expected number of steps for this procedure to terminate is $S_N$. We formalize this result as the following theorem:

\begin{theorem} \label{theorem:efficiency}
Assume that the position of a plan (after sampling-based validation) in the ordered plans with respect to their costs is uniformly distributed.
Let $N$ be the number of different join trees in the search space.
The expected number of steps before the re-optimization procedure terminates is then $S_N$, where $S_N$ is computed by Equation~\ref{eq:SN}.
Moreover, $S_N=O(\sqrt{N})$ by Theorem~\ref{theorem:SN-upper-bound}.
\end{theorem}

We emphasize that the analysis here only targets worst-case performance, which might be too pessimistic. This is because Procedure~\ref{procedure:random-ball-model} only simulates the Case (3) stated in Theorem~\ref{theorem:sequence-transformation}, which is the worst one among the three possible cases. In our experiments, we have found that all queries we tested require less than 10 rounds of iteration, most of which require only 1 or 2 rounds.

\blankline

\remark{The uniformity assumption in Theorem~\ref{theorem:efficiency} may not be valid in practice. It is possible that a plan after sampling-based validation (or, a marked ball in terms of Procedure~\ref{procedure:random-ball-model}) is more likely to be inserted into the front/back half of the queue. Such cases imply that, rather than with an equal chance of overestimation/underestimation, the optimizer tends to overestimate/underestimate the costs of all query plans (for a particular query). This is, however, not impossible.
In practice, significant cardinality estimation errors usually appear locally and propagate upwards. Once the error at some join were corrected, the errors in all plans that contain that join would also be corrected. In other words, the correction of the error at a single join can lead to the correction of errors in many candidate plans. In Appendix~\ref{appendix:sec:analysis}, we further present analysis for two extreme cases: all local errors are overestimates/underestimates. Any real case sits in between.
To summarize, for left-deep join trees, we have the following two results:
\begin{itemize}
\item If all local errors are overestimates, then in the worst case the re-optimization procedure would terminate in at most $m+1$ steps, where $m$ is the number of joins in the query.
\item If all local errors are underestimates, then in the worst case the re-optimization procedure is expected to terminate in $S_{N/M}$ steps, where $N$ is the number of different join trees in the optimizer's search space and $M$ is the number of edges in the join graph.
\end{itemize}
Note that both results are better than the bound stated in Theorem~\ref{theorem:efficiency}.
For instance, in the underestimation-only case, if $N=1000$ and $M=10$, we have $S_N=39$ but $S_{N/M}=12$.}

%\todo{We can challenge the assumption used in the probabilistic model by saying that the ball is more likely to be inserted at the front/back half of the queue. In general, we can assume an arbitrary distribution of the likelihoods that a ball could be inserted back into the positions of the queue. Then we can do a simulation (e.g., Monte Carlo experiments) to compute the number of steps before the procedure terminates.}


%\paragraph{Overestimates And Underestimates}
%
%It is more natural in practice that both overestimates and underestimates could occur. The expected number of steps before the re-optimization procedure terminates is then between that of the two extreme cases discussed above.

\subsection{Optimality of the Final Plan} \label{sec:analysis:optimality}

We can think of the re-optimization procedure as progressive adjustments of the optimizer's direction when it explores its search space. Of course, the search space depends on the algorithm or strategy used by the optimizer, and thus the impact of re-optimization also depends on that.
But we can still have some general conclusions about the optimality of the final plan regardless of the search space.

\begin{assumption}\label{assumption:cost-function}
The cost estimates of plans after using sampling-based cardinality refinement are consistent. That is, for any two plans $P_1$ and $P_2$, if $\cost^s(P_1) < \cost^s(P_2)$, then $\cost^a(P_1) < \cost^a(P_2)$. Here, $\cost^s(P)$ and $\cost^a(P)$ are the estimated cost based on sampling and the actual cost of plan $P$, respectively.
\end{assumption}

We have the following theorem based on Assumption~\ref{assumption:cost-function}. The proof is included in Appendix~\ref{appendix:sec:proofs:theorem:local-optimality}.

\begin{theorem}\label{theorem:local-optimality}
Let $P_1$, ..., $P_n$ be a series of plans generated during re-optimization. Then $\cost^s(P_n)\leq \cost^s(P_i)$, and thus, by Assumption~\ref{assumption:cost-function}, it follows that $\cost^a(P_n)\leq\cost^a(P_i)$, for $1\leq i \leq n - 1$.
\end{theorem}

That is, the plan after re-optimization is guaranteed to be better than the original plan. Nonetheless, it is difficult to conclude that the plans are improved monotonically, namely, in general it is not true that $\cost^s(P_{i+1})\leq\cost^s(P_i)$, for $1\leq i\leq n - 1$. However, we can prove that this is true if we only have overestimates (proof in Appendix~\ref{appendix:sec:proofs:corollary:local-optimality:overestimates}).

\begin{corollary} \label{corollary:local-optimality:overestimates}
Let $P_1$, ..., $P_n$ be a series of plans generated during re-optimization. If in the re-optimization procedure only overestimates occur, then $\cost^s(P_{i+1})\leq\cost^s(P_i)$ for $1\leq i\leq n-1$.
\end{corollary}

Our last result on the optimality of the final plan is in the sense that it is the best among all the plans that are local transformations of the final plan (proof in Appendix~\ref{appendix:sec:proofs:theorem:optimality-local-transformation}).

\begin{theorem}\label{theorem:optimality-local-transformation}
Let $P$ be the final plan returned by the re-optimization procedure. For any $P'$ such that $P'$ is a local transformation of $P$, it holds that $\cost^s(P)\leq\cost^s(P')$.
\end{theorem}
%Again note that this implies that the final plan is the best among all the plans that have the same join tree.

\subsection{Discussion}

We call the final plan returned by the re-optimization procedure the \emph{fixed point} with respect to the initial plan generated by the optimizer. According to Theorem~\ref{theorem:local-optimality}, this plan is a \emph{local optimum} with respect to the initial plan. Note that, if $\mathcal{P} = \{P_1, ..., P_n\}$ covers the whole search space, that is, any plan $P$ in the search space is covered by $\mathcal{P}$, then the locally optimal plan obtained is also globally optimal.

A natural question is then the impact of the initial plan. Intuitively, it seems that the initial plan can affect both the fixed point and the time it takes to converge to the fixed point. (Note that it is straightforward to prove that the fixed point must exist and be unique, with respect to the given initial plan.) There are also other related interesting questions. For example, if we start with two initial plans with similar cost estimates, would they converge to fixed points with similar costs as well? We leave all these problems as interesting directions for further investigation.

Moreover, the convergence of the re-optimization procedure towards a fixed point can also be viewed as a validation procedure of the costs of the plans $\mathcal{V}$ that can be covered by $\mathcal{P}=\{P_1, ..., P_n\}$. Note that $\mathcal{V}$ is a subset of the whole search space explored by the optimizer, and $\mathcal{V}$ is induced by $P_1$ --- the initial plan that is deemed as optimal by the optimizer. It is also interesting future work to study the relationship between $P_1$ and $\mathcal{V}$, especially how much of the complete search space can be covered by $\mathcal{V}$.


%\begin{algorithm}
%  \SetAlgoLined
%  \KwIn{$q$, a given SQL query}
%  \KwOut{$P_q$, query plan of $q$ after re-optimization}
%  \SetAlgoLined
%  $\Gamma \leftarrow \emptyset$\;
%  $P_0\leftarrow \Null$\;
%  $i\leftarrow 1$\;
%  \Repeat {no\ new\ statistics\ added\ to\ $\Gamma$} {
%    $P_i\leftarrow GetPlanFromOptimizer(\Gamma)$\;
%    \If{$P_i$ is the same as $P_{i-1}$} {
%        \textbf{break}\;
%    }
%    $\Delta_i\leftarrow GetCardinalityEstimatesBySampling(P_i)$\;
%    \If{$\cost(P_i)^{\sampling}\geq \cost(P_i)^{\optimizer}$} {
%        \textbf{break}\;
%    }
%
%    $\Gamma\leftarrow\Gamma\cup\Delta_i$\;
%    $i\leftarrow i + 1$\;
%  }
%  Let the final plan be $P_q$\;
%  \Return{$P_q$\;}
%  \caption{Sampling-based query re-optimization (conservative version)}
%\label{alg:reoptimization-conservative}
%\end{algorithm} 

==> benchmark-old.tex <==
\section{Optimizer Torture Test}\label{sec:benchmark}

Evaluating the effectiveness of a query optimizer is challenging.
As we mentioned in the introduction, query optimizers have to handle not only common cases but also difficult, corner cases.
In view of this, we conduct performance evaluation for both common cases and corner cases.
%We argue that such performance analysis should be conducted for ``average-case'' queries as as well as ``hard-case'' queries.
For the former, we use the TPC-H benchmark databases. For the latter, we focus on queries whose cardinalities are difficult to be accurately estimated by using histogram-based approaches. Specifically, we generate a special database as well as a special set of queries with controlled degree of data correlation. We call it ``optimizer torture test'' (OTT), given that our goal is to sufficiently challenge the cardinality estimation approaches used by current query optimizers.
We next describe the details of OTT.

%Current query optimizers make two assumptions when they estimate cardinalities for queries:
%\begin{enumerate}[(i)]
%\item \emph{Uniformity} --- values of attributes with no available statistics such as histograms are uniformly distributed;
%\item \emph{Attribute-Value-Independence} (AVI) --- distributions of values of different attributes are independent.
%\end{enumerate}
%
%We therefore create databases that violate these two assumptions. To attack (i), we use a skewed version of the TPC-H benchmark database~\cite{skewed-gen}. To attack (ii), we generate a special database as well as a special set of queries with controlled degree of data correlation. We call it ``optimizer torture test'' (OTT), given that our goal is to sufficiently challenge the AVI assumption underlying cardinality estimation approaches used by current query optimizers.
%We next describe the details of OTT.

\subsection{Design of the Database and Queries}\label{sec:benchmark:design}

%Our goal of the benchmark is two-fold. On one hand, the benchmark should present high data correlations to sufficiently challenge the AVI assumption underlying cardinality estimation approaches used by current query optimizers. On the other hand, the selectivity/cadinality of queries over the benchmark should be easy to estimate manually, so that we can understand and evaluate the experimental results fairly.

Since we target cardinality/selectivity estimation, we can focus on queries that only contain selections and joins.
In general, a selection-join query $q$ over $K$ relations $R_1$, ..., $R_K$ can be represented as
$$q=\sigma_{F}(R_1\bowtie\cdots\bowtie R_K),$$
where $F$ is a selection predicate as in relational algebra (i.e., a boolean formula).
Moreover, we can just focus on equality predicates, i.e., predicates of the form $A=c$ where $A$ is an attribute and $c$ is a constant. Any other predicate can be represented by unions of equality predicates. As a result, we can focus on $F$ of the form
$$F=(A_1=c_1)\land \cdots\land (A_K=c_K),$$
where $A_k$ is an attribute of $R_k$, and $c_k\in\Dom(A_k)$ ($1\leq k\leq K$). Here, $\Dom(A_k)$ is the domain of the attribute $A_k$.

Based on these observations, our design of the database and queries is as follows:
\begin{enumerate} [(1)]
\item We have $K$ relations $R_1(A_1, B_1)$, ..., $R_K(A_K, B_K)$.
\item We use $A_k$'s for selections and $B_k$'s for joins.
\item Let $R'_k=\sigma_{A_k=c_k}(R_k)$ for $1\leq k\leq K$.
The queries of our benchmark are then of the form:
\begin{equation}\label{eq:query}
R'_1\bowtie_{B_1=B_2}R'_2\bowtie_{B_2=B_3}\cdots\bowtie_{B_{K-1}=B_K}R'_K.
\end{equation}
\end{enumerate}

The remaining question is how to generate data for $R_1$, ..., $R_K$ so that we can easily control the selectivities for the selection and join predicates. This requires us to consider the joint data distribution for $(A_1, ..., A_K, B_1, ..., B_K)$. A straightforward way could be to specify the contingency table of the distribution. However, there is a subtle issue of this approach: we cannot just generate a large table with attributes $A_1$, ..., $A_K$, $B_1$, ..., $B_K$ and then split it into different relations $R_1(A_1, B_1)$, ..., $R_K(A_K, B_K)$. To see why this is incorrect, let us consider the following example.

\begin{example}[Approach Using Joint Distribution]\label{example:distribution}
Suppose that we need to generate binary values for two attributes $A_1$ and $A_2$, with the following joint distribution:
\begin{enumerate}[(1)]
\item $p_{00}=\Pr(A_1=0, A_2=0)=0.1$;
\item $p_{01}=\Pr(A_1=0, A_2=1)=0$;
\item $p_{10}=\Pr(A_1=1, A_2=0)=0$;
\item $p_{11}=\Pr(A_1=1, A_2=1)=0.9$.
\end{enumerate}
Assume that we generate 10 tuples $(A_1, A_2)$ according to the above distribution. Then we would expect to obtain a multiset of tuples: $\{1\cdot(0,0),9\cdot(1,1)\}$. Here the notation $1\cdot(0,0)$ means there is one $(0,0)$ in the multiset. If we project the tuples onto $A_1$ and $A_2$ (without removing duplicates), we have $A_1=A_2=\{1\cdot 0, 9\cdot 1\}$. Now what is the joint distribution of $(A_1, A_2)$ once we see such a database? Note that we have no idea about the \emph{true} joint distribution that governs the generation of the data, because we are only allowed to see the \emph{marginal} distributions of $A_1$ and $A_2$. A natural inference of the joint distribution could be to consider the cross product $A_1\times A_2$. In this case we have
\begin{eqnarray*}
A_1\times A_2 &=& \{1\cdot 0, 9\cdot 1\}\times\{1\cdot 0, 9\cdot 1\}\\
&=& \{1\cdot(0,0), 9\cdot(0,1), 9\cdot(1,0), 81\cdot(1,1)\}.
\end{eqnarray*}
Hence, the ``observed'' joint distribution of $A_1$ and $A_2$ is:
\begin{enumerate}[(1)]
\item $p'_{00}=\Pr'(A_1=0, A_2=0)=1/100=0.01$;
\item $p'_{01}=\Pr'(A_1=0, A_2=1)=9/100=0.09$;
\item $p'_{10}=\Pr'(A_1=1, A_2=0)=9/100=0.09$;
\item $p'_{11}=\Pr'(A_1=1, A_2=1)=81/100=0.81$.
\end{enumerate}
\end{example}

The ``observed'' joint distribution is indeed ``the'' joint distribution when tables are joined. It might be easier to see this if we rewrite the query in Equation~\ref{eq:query} as
\begin{equation}\label{eq:query2}
\sigma_{A_1=c_1\land\cdots \land A_K=c_K\land B_1=B_2\land\cdots\land B_{K-1}=B_K}(R_1\times\cdots\times R_K).
\end{equation}
The previous example shows that there is information loss when marginalizing out attributes, which is somewhat similar to the notion of lossless/lossy joins in database normalization theory.
This discrepancy between the true and observed joint distributions calls for a new approach.

\subsection{The Data Generation Algorithm} \label{sec:benchmark:data-gen}

The previous analysis suggests that we can only generate data for each $R_k(A_k, B_k)$ separately and independently, without resorting to their joint distribution. To generate correlated data, we therefore have to make $A_k$ and $B_k$ correlated, for $1\leq k\leq K$.
Because our goal is to challenge the optimizer's cardinality estimation algorithm, we choose to go to the extreme of this direction: let $B_k$ be the same as $A_k$. Algorithm~\ref{alg:data-gen} presents the details of this idea.

\begin{algorithm}
  \SetAlgoLined
  \KwIn{$\Pr(A_k)$, the distribution of $A_k$, for $1\leq k\leq K$}
  \KwOut{$R_k(A_k,B_k)$: tables generated, for $1\leq k\leq K$}
  \SetAlgoLined
  \For{$1\leq k\leq K$} {
    Pick a seed independently for the random number generator\;
    Generate $A_k$ with respect to $\Pr(A_k)$\;
    Generate $B_k=A_k$\;
  }
  \Return{$R_k(A_k,B_k)$, $1\leq k\leq K$\;}
  \caption{Data generation for the OTT database}
\label{alg:data-gen}
\end{algorithm}

We are left with the problem of specifying $\Pr(A_k)$. While $\Pr(A_k)$ could be arbitrary, we should reconsider our goal of sufficiently challenging the optimizer. We therefore need to know some details about how the optimizer estimates selectivities/cardinalities. Of course, different query optimizers have different implementations, but the general principles are similar. % they use statistics (usually histograms) and rely on the AVI assumption.
In the following, we present the specific technique used by PostgreSQL, which is used in our experimental evaluation in Section~\ref{sec:experiments}.

\subsubsection{PostgreSQL's Approaches} \label{sec:benchmark:data-gen:postgresql}

PostgreSQL stores the following three types of statistics for each attribute $A$ in its \verb|pg_stats| view~\cite{pg-stats}, if the \verb|ANALYZE| command is invoked for the database:
\begin{itemize}
\item the number of distinct values $n(A)$ of $A$;
\item a list of most common values (MCV's) of $A$ and their frequency;
\item an equal-depth histogram for the other values of $A$ except for the MCV's.
\end{itemize}

The above statistics can be used to estimate the selectivity of a predicate over a single attribute in a straightforward manner.
For instance, for the predicate $A=c$ in our OTT queries, PostgreSQL would first check if $c$ is in the MCV's.
If $c$ is present, then the optimizer simply uses the (exact) frequency recorded.
Otherwise, the optimizer assumes a uniform distribution over the non-MCV's and estimates the frequency of $c$ based on $n(A)$.

The approach used by PostgreSQL to estimate selectivities for join predicates is more sophisticated. Consider an equal-join predicate $B_1=B_2$. If MCV's for either $B_1$ or $B_2$ are not available, then the optimizer uses an approach first introduced in System R~\cite{Selinger-AccessPath79} by estimating the reduction factor as $1/\max\{n(B_1),n(B_2)\}$. If, on the other hand, MCV's are available for both $B_1$ and $B_2$, then PostgreSQL tries to refine its estimate by first ``joining'' the two lists of MCV's. For skewed data distributions, this can lead to much better estimates because the join size of the MCV's, which is accurate, would be very close to the actual join size. Other database systems, such as Oracle~\cite{oracle-join-est}, use similar approaches.

To combine selectivities from multiple predicates, PostgreSQL relies on the attribute-value-independence (AVI) assumption, which assumes that the distributions of values of different attributes are independent.
%For example, PostgreSQL simply estimates the selectivity of a conjunction of predicates as the product of the selectivities of individual predicates.

\subsubsection{The Distribution $\Pr(A_k)$ And Its Impact}

From the previous discussion we can see that whether $\Pr(A_k)$ is uniform or skewed would have little difference in affecting the optimizer's estimates if MCV's were leveraged, simply because MCV's have recorded the \emph{exact} frequency for those skewed values. We therefore can just let $\Pr(A_k)$ be uniform. We next analyze the impact of this decision by computing the differences between the estimated and actual cardinalities for the OTT queries.

Let us first revisit the OTT queries presented in Equation~\ref{eq:query}. Note that for an OTT query to be non-empty, the following condition must hold: $B_1=B_2=\cdots =B_{K-1}=B_K$. Because we have intentionally set $A_k=B_k$ for $1\leq k\leq K$, this then implies
\begin{equation} \label{eq:non-empty-condition}
A_1=A_2=\cdots =A_{K-1}=A_K.
\end{equation}
The query size can thus be controlled by the values of the $A$'s. The query is simply empty if Equation~\ref{eq:non-empty-condition} does not hold. We now compute the query size when Equation~\ref{eq:non-empty-condition} holds.

Consider a specific query $q$ where the constants in the selection predicates are fixed. Let us compute the cardinality of $q$, which is equivalent to computing the selectivity of the predicate in Equation~\ref{eq:query2}. In probabilistic sense, the selectivity $s$ can be interpreted as the chance that a (randomly picked) tuple from $R_1\times\cdots\times R_K$ making the selection predicate true. That is,
$$s=\Pr(A_1=c_1, \cdots, A_K=c_K, B_1=\cdots=B_K).$$

\begin{lemma}\label{lemma:s-actual}
When Equation~\ref{eq:non-empty-condition} holds, we have
$$s=\prod\nolimits_{k=1}^{K}\frac{1}{n(A_k)}.$$
\end{lemma}

The proof is included in Appendix~\ref{appendix:sec:proofs:lemma:s-actual}. As a result, the join size of $q$ is
$$|q|=s\cdot \prod\nolimits_{k=1}^K|R_k|=\prod\nolimits_{k=1}^K\frac{|R_k|}{n(A_k)}.$$
To summarize, we have
\begin{displaymath}
|q|=\left\{
\begin{array}{ll}
\prod\nolimits_{k=1}^K\frac{|R_k|}{n(A_k)}, & \textrm{if $c_1=\cdots =c_K$;}\\
0, & \textrm{otherwise.}
\end{array}
\right.
\end{displaymath}

Now what would be the query size estimated by the optimizer? Again, let us compute the estimated selectivity $\hat{s}$, assuming that the optimizer knows the exact histograms of the $A_k$ and $B_k$ ($1\leq k\leq K$). Note that this assumption is stronger than the case in Section~\ref{sec:benchmark:data-gen:postgresql}, where the optimizer possesses exact histograms only for MCV's.
%Furthermore, to ease our computation, we assume that $\Dom(B_k)$ is the same for $1\leq k\leq K$.
We then have the following result:

\begin{lemma}\label{lemma:s-estimated}
Suppose that the AVI assumption is used. Assuming that $\Dom(B_k)$ is the same for $1\leq k\leq K$ and $|\Dom(B_k)|=L$, we have
$$\hat{s}=\frac{1}{L^{K-1}}\prod\nolimits_{k=1}^{K}\frac{1}{n(A_k)}.$$
\end{lemma}

The proof is included in Appendix~\ref{appendix:sec:proofs:lemma:s-estimated}.
Hence, the estimated size of $q$ is
$$\widehat{|q|}=\hat{s}\cdot \prod\nolimits_{k=1}^K|R_k|=\frac{1}{L^{K-1}}\prod\nolimits_{k=1}^K\frac{|R_k|}{n(A_k)}.$$
Note that this is regardless of if Equation~\ref{eq:non-empty-condition} holds or not.

Comparing the expressions of $|q|$ and $\widehat{|q|}$, if we define
$$d=\mid|q|-\widehat{|q|}\mid,$$
it then follows that
\begin{displaymath}
d=\left\{
\begin{array}{ll}
\big(1-\frac{1}{L^{K-1}}\big)\cdot\prod\nolimits_{k=1}^K\frac{|R_k|}{n(A_k)}, & \textrm{if $c_1=\cdots =c_K$;}\\
\frac{1}{L^{K-1}}\cdot\prod\nolimits_{k=1}^K\frac{|R_k|}{n(A_k)}, & \textrm{otherwise.}
\end{array}
\right.
\end{displaymath}

Let us further get some intuition about how large $d$ could be by considering the following specific example.
\begin{example}
For simplicity, assume that $M=|R_k| / n(A_k)$ is the same for $1\leq k\leq K$. $M$ is then the number of tuples per distinct value of $A_k$ ($1\leq k\leq K$). In this case,
\begin{displaymath}
d=\left\{
\begin{array}{ll}
\big(1- 1 / L^{K-1}\big)\cdot M^K, & \textrm{if $c_1=\cdots =c_K$;}\\
M^K / L^{K-1}, & \textrm{otherwise.}
\end{array}
\right.
\end{displaymath}
If $L=100$ and $M=100$, it then follows that
\begin{displaymath}
d=\left\{
\begin{array}{ll}
100^K - 100, & \textrm{if $c_1=\cdots =c_K$;}\\
100, & \textrm{otherwise.}
\end{array}
\right.
\end{displaymath}
For $K=4$ (i.e., just 3 joins), $d\approx 10^8$ if it happens to be that $c_1=\cdots =c_K$.
Moreover, if $c_1=\cdots =c_K$, then $|q|>\widehat{|q|}$.
Therefore, the optimizer would significantly underestimate the size of the join (by $10^8$).
So it is likely that the optimizer would pick an inefficient plan that it thought were efficient.
\end{example}

%\subsubsection{Discussion}



==> benchmarkBackup.tex <==
\subsection{The Case of Two Binary Attributes}

For ease of exposition, let us still focus on the case of two binary attributes $A_1$ and $A_2$. Our question is: how can we generate values for $A_1$ and $A_2$ so that the observed distribution matches the specified one? We next give a formulation of this problem.

\begin{theorem}\label{theorem:match}
In the case of two binary attributes, if the observed joint distribution matches the actual one, then
$$p_{00}\cdot p_{11}=p_{01}\cdot p_{10}.$$
\end{theorem}
\begin{proof}
Suppose that $A_1=\{x_1\cdot 0, y_1\cdot 1\}$ and $A_2=\{x_2\cdot 0, y_2\cdot 1\}$. Define $n_1=x_1x_2$, $n_2=x_1y_2$, $n_3=x_2y_1$, and $n_4=y_1y_2$. We have the observed joint distribution for $(A_1, A_2)$:
\begin{enumerate}[(1)]
\item $p'_{00}=\Pr'(A_1=0, A_2=0)=n_1/(n_1+n_2+n_3+n_4)$;
\item $p'_{01}=\Pr'(A_1=0, A_2=1)=n_2/(n_1+n_2+n_3+n_4)$;
\item $p'_{10}=\Pr'(A_1=1, A_2=0)=n_3/(n_1+n_2+n_3+n_4)$;
\item $p'_{11}=\Pr'(A_1=1, A_2=1)=n_4/(n_1+n_2+n_3+n_4)$.
\end{enumerate}
To let the observed distribution match the actual one, we must have $p'_{00}=p_{00}$, $p'_{01}=p_{01}$, $p'_{10}=p_{10}$, and $p'_{11}=p_{11}$. It follows that
\begin{displaymath}
\left\{
\begin{array}{l}
n_1=p_{00}\cdot (n_1+n_2+n_3+n_4)\\
n_2=p_{01}\cdot (n_1+n_2+n_3+n_4)\\
n_3=p_{10}\cdot (n_1+n_2+n_3+n_4)\\
n_4=p_{11}\cdot (n_1+n_2+n_3+n_4).
\end{array}
\right.
\end{displaymath}
Solving this linear system of equations we have
\begin{displaymath}
\left\{
\begin{array}{l}
n_1=(p_{00}/p_{11})\cdot n_4\\
n_2=(p_{01}/p_{11})\cdot n_4\\
n_3=(p_{10}/p_{11})\cdot n_4,
\end{array}
\right.
\end{displaymath}
which further implies that
\begin{displaymath}
\left\{
\begin{array}{l}
x_1x_2=(p_{00}/p_{11})\cdot y_1y_2\\
x_1=(p_{01}/p_{11})\cdot y_1\\
x_2=(p_{10}/p_{11})\cdot y_2.
\end{array}
\right.
\end{displaymath}
Therefore, it follows that $p_{00}\cdot p_{11}=p_{01}\cdot p_{10}$, which completes the proof of the theorem.
\end{proof}

It is now easy to see why the distribution in Example~\ref{example:distribution} is infeasible: the necessary condition stated in Theorem~\ref{theorem:match} does not hold. It is also straightforward to figure out $x_1$, $y_1$, $x_2$, and $y_2$ once $|A_1|$ and $|A_2|$ are given. We have
\begin{displaymath}
\left\{
\begin{array}{l}
x_1+y_1 = |A_1|\\
x_2+y_2 = |A_2|\\
x_1=(p_{01}/p_{11})\cdot y_1\\
x_2=(p_{10}/p_{11})\cdot y_2.
\end{array}
\right.
\end{displaymath}
As a result, it follows that
\begin{displaymath}
\left\{
\begin{array}{l}
x_1 = (p_{01} / (p_{01}+p_{11}))\cdot |A_1|\\
y_1 = (p_{11} / (p_{01}+p_{11}))\cdot |A_1|\\
x_2 = (p_{10} / (p_{10}+p_{11}))\cdot |A_2|\\
y_2 = (p_{11} / (p_{10}+p_{11}))\cdot |A_2|.
\end{array}
\right.
\end{displaymath}

Therefore, the key to data generation is specifying the true distribution with respect to the constraint stated in Theorem~\ref{theorem:match}. A remaining question is if we can generate skewed distribution given that constraint. We give some further analysis of this.

\begin{theorem}\label{theorem:skew}
Suppose that $p_{11}>0$ is given. Then $p_{00}$ achieves its maximum $p_{00}^{\max}$ when $p_{01}=p_{10}$, where  $p_{00}^{\max}=(\sqrt{p_{11}}-1)^2$.
\end{theorem}

\begin{proof}
The system of constraints that the joint distribution should satisfy is now:
\begin{displaymath}
\left\{
\begin{array}{l}
p_{00}+p_{01}+p_{10}+p_{10}+p_{11}=1\\
p_{00}\cdot p_{11}=p_{01}\cdot p_{10}.
\end{array}
\right.
\end{displaymath}
Let $x=p_{01}+p_{10}$ and $y=p_{01}\cdot p_{10}$. We then have
\begin{displaymath}
\left\{
\begin{array}{l}
x=1-(p_{00}+p_{11})\\
y=p_{00}\cdot p_{11}.
\end{array}
\right.
\end{displaymath}
Since $4y\leq x^2$, where the equality holds if and only if $p_{01}=p_{10}$, it follows that
$$\big(1-(p_{00}+p_{11})\big)^2\geq 4p_{00}p_{11}.$$
This is equivalent to
$$\big(p_{00}-p_{11}-1\big)^2\geq 4p_{11}.$$
Therefore, either $p_{00}\geq(\sqrt{p_{11}}+1)^2$ or $p_{00}\leq(\sqrt{p_{11}}-1)^2$.
However, since $p_{11}>0$, the former implies $p_{00}>1$, which is impossible.
As a result, we must have $p_{00}\leq(\sqrt{p_{11}}-1)^2$.
Hence, $p_{00}$ achieve its maximum when $p_{01}=p_{10}$.
This completes the proof of the theorem.
\end{proof}

Note that Theorem~\ref{theorem:skew} only requires that $p_{11}>0$.
This implies that we can create arbitrarily skewed data.
As an example, suppose that $p_{11}=0.0001$.
Then $p_{00}^{\max}=0.9801$, which is achieved when $p_{01}=p_{10}=9.9\times 10^{-3}$.
In fact, we can even let $p_{11}=0$. Then $p_{00}^{\max}=1$ when $p_{01}=p_{10}=0$, though this seems too trivial.

\subsection{The Data Generation Algorithm}

The solution from the previous section could quickly mess things up if we consider the general case where we have $n$ multi-valued attributes. Although the same idea applies, figuring out the details is complicated and tedious. For the purpose of this paper, we argue that it is sufficient to focus ourselves on pairwise joint distributions of binary attributes. The reason is that we only need various degrees of skewness, which could be captured by specifying different contingency tables. Table~\ref{tab:contingency-table} gives an example contingency table.

\begin{table}[th]
\small
\centering
\begin{tabular}{|l|r|r|r|}
  \hline
$A_1$ / $A_2$& $0$ & $1$ & $\Pr(A_1)$ \\
\hline
$0$ & $0.9801$ & $9.9\times 10^{-3}$ & $0.99$\\
$1$ & $9.9\times 10^{-3}$ & $0.0001$ & $0.01$\\
\hline
$\Pr(A_2)$ & $0.99$ & $0.01$ & $1.0$\\
  \hline
\end{tabular}
\caption{Example contingency table}
\label{tab:contingency-table}
\shrink
\end{table}

Specifically, our data generation algorithm works as follows. Our database contains $2K$ tables $R_1$, ..., $R_{2K}$. As before, each table is of the form $R_k(A_k, B_k)$ ($1\leq k\leq 2K$), and all the attributes are binary. Moreover, we require $B_k=A_k$ ($1\leq k\leq 2K$). For each pair of attributes $A_{2i-1}$ and $A_{2i}$, we specify a contingency table that represents the joint distribution of $(A_{2i-1}, A_{2i})$ ($1\leq i\leq K$), and generate data based on the approach presented in the previous section. However, we do not specify joint distributions for the other pairs of attributes, i.e., we assume that they are pairwise independent. We do this by simply using a randomly picked seed for the random number generator each time we generate $A_{2i-1}$. \todo{Is this correct?}

\begin{algorithm}
  \SetAlgoLined
  \KwIn{$T_i$, the contingency table of $(A_{2i-1}, A_{2i})$, for $1\leq i\leq K$}
  \KwOut{$R_k(A_k,B_k)$: tables generated, for $1\leq k\leq 2K$}
  \SetAlgoLined
  \For{$1\leq i\leq K$} {
    Randomly pick a seed for the random number generator\;
    Generate $A_{2i-1}$ with respect to $x_{2i-1}$ and $y_{2i-1}$ based on $T_i$ and $|A_{2i-1}|$\;
    Generate $B_{2i-1}=A_{2i-1}$\;
    Generate $A_{2i}$ with respect to $x_{2i}$ and $y_{2i}$ based on $T_i$ and $|A_{2i}|$\;
    Generate $B_{2i}=A_{2i}$\;
  }
  \Return{$R_k(A_k,B_k)$, $1\leq k\leq 2K$\;}
  \caption{Data generation}
\label{alg:data-gen}
\end{algorithm}

We now illustrate how we can control selectivities of selection-join queries with the particular form described in Equation~(\ref{eq:query}).

Consider a specific query where the constants in the selection predicates are fixed (i.e., they are either 0 or 1).
Let us compute the cardinality of this query, which is equivalent to computing the selectivity of the predicate in Equation~(\ref{eq:query2}). In probabilistic sense, the selectivity $s$ can be interpreted as the chance that a (randomly picked) tuple from $R_1\times\cdots\times R_{2K}$ making the selection predicate true. That is,
$$s=\Pr(A_1=c_1, \cdots, A_{2K}=c_{2K}, B_1=B_2,\cdots, B_{2K-1}=B_{2K}),$$
or equivalently,
\begin{eqnarray*}
s&=&\Pr(B_1=B_2,\cdots, B_{2K-1}=B_{2K}|A_1=c_1, \cdots , A_{2K}=c_{2K})\\
&\times &\Pr(A_1=c_1, \cdots , A_{2K}=c_{2K}).
\end{eqnarray*}

Let $\Pr(\mathbf{B}|\mathbf{A})=\Pr(B_1=B_2,\cdots, B_{2K-1}=B_{2K}|A_1=c_1, \cdots , A_{2K}=c_{2K})$, and $\Pr(\mathbf{A})=\Pr(A_1=c_1, \cdots , A_{2K}=c_{2K})$.
Since $B_k=A_k$ ($1\leq k\leq 2K$), $\Pr(\mathbf{B}|\mathbf{A})$ equals either 0 or 1, depending on the specific values of $c_1$, ..., $c_{2K}$.
Moreover, $\Pr(\mathbf{B}|\mathbf{A})=1$ if and only if $c_1=c_2$, ..., $c_{2K-1}=c_{2K}$. We therefore have
\begin{displaymath}
s=\left\{
\begin{array}{ll}
\Pr(\mathbf{A}), & \textrm{if $c_1=c_2$, ..., $c_{2K-1}=c_{2K}$;}\\
0, & \textrm{otherwise.}
\end{array}
\right.
\end{displaymath}
Now consider $\Pr(\mathbf{A})$. Based on our design, only $A_{2i-1}$ and $A_{2i}$ are dependent ($1\leq i\leq K$). As a result, we have
$$\Pr(\mathbf{A})=\prod_{i=1}^K\Pr(A_{2i-1}=c_{2i-1}, A_{2i}=c_{2i}).$$

We next compute the selectivity $s'$ if we rely on the AVI assumption for cardinality estimation. We have
$$s'=\prod_{k=1}^{2K}\Pr(A_k=c_k)\prod_{i=1}^{K}\Pr(B_{2i-1}=B_{2i}).$$
Based on the classic approach (used in System R),
$$\Pr(B_{2i-1}=B_{2i})=\frac{1}{\max\{d(B_{2i-1}), d(B_{2i})\}},$$
where $d(A)$ is the number of distinct values in the attribute $A$.
Since all attributes are binary, we have $\Pr(B_{2i-1}=B_{2i})=1/2$.
Therefore, we have
$$s'=\big(\frac{1}{2}\big)^K\cdot\prod_{i=1}^{K}\Pr(A_{2i-1}=c_{2i-1})\Pr(A_{2i}=c_{2i}).$$

Let us define the relative error to be $E=\frac{|s'-s|}{s'}$. Based on the previous analysis, we have
\begin{displaymath}
E=\left\{
\begin{array}{ll}
\big|1 - 2^K\cdot\prod_{i=1}^K\frac{p(c_{2i-1}, c_{2i})}{p(c_{2i-1})p(c_{2i})}\big|, & \textrm{if $c_{2i-1}=c_{2i}$;}\\
1, & \textrm{otherwise.}
\end{array}
\right.
\end{displaymath}
Here we have used $p(c_1, c_2)$ for $\Pr(A_1=c_1, A_2=c_2)$. However, if the condition stated in Theorem~\ref{theorem:match} must hold, then independence is implied, as we show next.

\begin{theorem}
If $p_{00}\cdot p_{11}=p_{01}\cdot p_{10}$, then $\Pr(A_1, A_2)=\Pr(A_1)\cdot \Pr(A_2)$.
\end{theorem}

\begin{proof}
Consider $\Pr(A_1=0)$ and $\Pr(A_2=0)$. For notational convenience, we use $\pi_i(j)$ for $\Pr(A_i)=j$. We then have $\pi_1(0)=\Pr(A_1=0)=p_{00}+p_{01}$ and $\pi_2(0)=\Pr(A_2=0)=p_{00}+p_{10}$.
Thus,
\begin{eqnarray*}
\pi_1(0)\pi_2(0)&=&(p_{00}+p_{01})(p_{00}+p_{10})\\
&=&p_{00}(p_{00}+p_{01}+p_{10}) + p_{01}p_{10}\\
&=&p_{00}(p_{00}+p_{01}+p_{10}) + p_{00}p_{11}\\
&=&p_{00}(p_{00}+p_{01}+p_{10}+p_{11})\\
&=&p_{00}.
\end{eqnarray*}
Similarly, we have
\begin{eqnarray*}
\pi_1(1)\pi_2(0)&=&(p_{10}+p_{11})(p_{00}+p_{10})\\
&=&p_{10}(p_{00}+p_{10}+p_{11}) + p_{00}p_{11}\\
&=&p_{10}(p_{00}+p_{10}+p_{11}) + p_{01}p_{10}\\
&=&p_{10}(p_{00}+p_{01}+p_{10}+p_{11})\\
&=&p_{10}.
\end{eqnarray*}
Therefore,
\begin{eqnarray*}
\pi_1(0)\pi_2(1)&=&\Pr(A_1=0)(1-\Pr(A_2=0))\\
&=&\Pr(A_1=0)-\Pr(A_1=0)\Pr(A_2=0)\\
&=&\Pr(A_1=0)-\Pr(A_1=0, A_2=0)\\
&=&\Pr(A_1=0)-\Pr(A_2=0|A_1=0)\Pr(A_1=0)\\
&=&(1-\Pr(A_2=0|A_1=0))\Pr(A_1=0)\\
&=&\Pr(A_2=1|A_1=0)\Pr(A_1=0)\\
&=&\Pr(A_1=0,A_2=1)=p_{01}.
\end{eqnarray*}
And similarly,
\begin{eqnarray*}
\pi_1(1)\pi_2(1)&=&\Pr(A_1=1)(1-\Pr(A_2=0))\\
&=&\Pr(A_1=1)-\Pr(A_1=1)\Pr(A_2=0)\\
&=&\Pr(A_1=1)-\Pr(A_1=1, A_2=0)\\
&=&\Pr(A_1=1)-\Pr(A_2=0|A_1=1)\Pr(A_1=1)\\
&=&(1-\Pr(A_2=0|A_1=1))\Pr(A_1=1)\\
&=&\Pr(A_2=1|A_1=1)\Pr(A_1=1)\\
&=&\Pr(A_1=1,A_2=1)=p_{11}.
\end{eqnarray*}
This completes the proof of the theorem.
\end{proof}

Therefore, we have $p(c_{2i-1}, c_{2i})=p(c_{2i-1})p(c_{2i})$. As a result,
\begin{displaymath}
E=\left\{
\begin{array}{ll}
2^K - 1, & \textrm{if $c_{2i-1}=c_{2i}$;}\\
1, & \textrm{otherwise.}
\end{array}
\right.
\end{displaymath}
The \emph{absolute} error in selectivity estimate is thus
\begin{displaymath}
|s-s'|= E\cdot s'=\left\{
\begin{array}{ll}
(2^K-1)s', & \textrm{if $c_{2i-1}=c_{2i}$;}\\
s', & \textrm{otherwise.}
\end{array}
\right.
\end{displaymath}
If we further consider the difference in terms of cardinality, then
\begin{displaymath}
d=|s-s'|\cdot|\mathbf{R}|=\left\{
\begin{array}{ll}
(2^K-1)s'|\mathbf{R}|, & \textrm{if $c_{2i-1}=c_{2i}$;}\\
s'|\mathbf{R}|, & \textrm{otherwise.}
\end{array}
\right.
\end{displaymath}
Here, $|\mathbf{R}|=\prod_{k=1}^{2K}|R_k|$. Let us further define $S_k=\Pr(A_k=c_k)|R_k|$. Then
\begin{displaymath}
d=\left\{
\begin{array}{ll}
(1-\frac{1}{2^K})\prod_{k=1}^{2K}S_k, & \textrm{if $c_{2i-1}=c_{2i}$;}\\
\frac{1}{2^K}\prod_{k=1}^{2K}S_k, & \textrm{otherwise.}
\end{array}
\right.
\end{displaymath}
Therefore, the cardinality estimation error is exponentially growing with respect to $K$.
If all relations have at least $10^4$ tuples, for example, then $d$ is at least $(5\times 10^7)^K$, a huge number even for $K=1$.


\paragraph*{Remark}

We would like to note here that the contingency table actually has no impact on the correlations between different attributes: it only controls \emph{skewness} of the marginal distributions.
This is somewhat surprising and counterintuitive.
However, we would realize that this is true once we understood the subtle point of ``implied data independence'' as mentioned before.
This is an inherent problem given that we have to generate the relations individually: the joint distribution information is lost when we separate values into different attributes.
Now that different join attributes are independent, an interesting question is then where data correlation does come from.
The answer is that data correlation is only subsumed by the dependency between attributes inside each relation.
In our case, we have forced $A_k=B_k$ and we actually use the $A_k$'s to control the $B_k$'s.
In other words, while $\Pr(\mathbf{B})=\prod_{k=1}^{2K}\Pr(B_k)$, $\Pr(\mathbf{B}|\mathbf{A})\neq\prod_{k=1}^{2K}\Pr(B_k|\mathbf{A})$.
We argue that this is the only source that data correlation can be from, if we want to generate relations individually (i.e., without any constraints such as functional dependency).
But, as we have shown, we can still observe huge errors in selectivity estimates by just utilizing the skewness of the $A_k$'s.

==> experiments-old.tex <==
\section{Experimental Evaluation} \label{sec:experiments}

We present experimental evaluation results of our proposed re-optimization procedure in this section.

\subsection{Experimental Settings} \label{sec:experiments:settings}

We implemented our proposed re-optimization framework in PostgreSQL 9.0.4. The modification to the optimizer is small, limited to several hundred lines of C code, which demonstrates the feasibility of including our framework into current query optimizers. We conducted our experiments on a PC configured with 2.4GHz Intel dual-core CPU and 4GB memory, and we ran PostgreSQL under Linux 2.6.18.

\subsubsection{Databases and Performance Metrics}

As mentioned before, we used both the standard version and a skewed version~\cite{skewed-gen} of the TPC-H benchmark database, as well as our own OTT database described in Section~\ref{sec:benchmark}. %We name our own benchmark as the ``HDC benchmark'' given its high data correlation.

\paragraph*{TPC-H Benchmark Databases}

We used 10GB TPC-H databases in our experiments.
The generator for skewed TPC-H database uses a parameter $z$ to control the skewness of each column by generating Zipfian distributions.
The larger $z$ is, the more skewed the generated data are.
$z=0$ corresponds to a uniform distribution.
%In our experiments, we generated databases by setting $z$ to be $0$, $1$, and $2$.
In our experiments, we generated a skewed database by setting $z=1$.

\paragraph*{OTT Database}

We created a specific instance of the OTT database in the following manner. We first generated a standard 1GB TPC-H database. We then extended the 6 largest tables (\emph{lineitem}, \emph{orders}, \emph{partsupp}, \emph{part}, \emph{customer}, \emph{supplier}) by adding two additional columns $A$ and $B$ to each of them. %\footnote{We do not use the two tiny tables \emph{nation} and \emph{region}.}
As discussed in Section~\ref{sec:benchmark:data-gen}, we populated the extra columns with uniform data.
The domain of a column is determined by the number of rows in the corresponding table: if the table contains $r$ rows, then the domain is $\{0, 1, ..., r / 100 - 1\}$. In other words, each distinct value in the domain would appear roughly 100 times in the generated column.
We further created an index on each added column.

\paragraph*{Performance Metrics}

We measured the following performance metrics for each query on each database:
\begin{enumerate} [(1)]
\item the original running time of the query;
\item the number of iterations the re-optimization procedure requires before its termination;
\item the time spent on the re-optimization procedure;
\item the total running time of the query including the re-optimization time.
\end{enumerate}
Based on studies in our previous work~\cite{WuCZTHN13}, in all of our experiments we set the sampling ratio to be 0.05, namely, $5\%$ of the data were taken as samples.

\subsubsection{Calibrating Cost Models}

In our previous work~\cite{WuCZTHN13}, we have also shown that, after proper calibration of the cost models used by the optimizer, we could have better estimates of query running times.
An interesting question is then: would calibration also help with query optimization?

In our experiments, we also investigated this problem.
Specifically, we ran the offline calibration procedure (details in~\cite{WuCZTHN13}) and replaced the default values of the five cost units (\emph{seq\_page\_cost}, \emph{random\_page\_cost}, \emph{cpu\_tuple\_cost}, \emph{cpu\_index\_tuple\_cost}, \emph{cpu\_operator\_cost}) in  \verb|postgresql.conf| (i.e., the configuration file of PostgreSQL server) with the calibrated values.
In the following, we also report results based on calibrated cost models.

\subsection{Results on the TPC-H Benchmark}

We tested 21 TPC-H queries. (We excluded Q15, which is not supported by our current implementation because it requires to create a view first.) For each TPC-H query, we randomly generated 10 instances. We cleared both the database buffer pool and the file system cache between each run of each query.

\subsubsection{Results on Uniform Database}

Figure~\ref{fig:tpch-skew0:time} presents the average running times and their standard deviations (as error bars) of these queries over the uniform database.

\begin{figure}[t]
\centering
\subfigure[Without calibration of the cost units]{ \label{fig:tpch-skew0:time:no-calib}
\includegraphics[width=\columnwidth]{./figs/reopt-new-join-only-with-dev-skew0-time-no-calib.eps}}
\subfigure[With calibration of the cost units]{ \label{fig:tpch-skew0:time:calib}
\includegraphics[width=\columnwidth]{./figs/reopt-new-join-only-with-dev-skew0-time-calib.eps}}
\caption{Query running time over uniform 10GB TPC-H database ($z=0$).}
\label{fig:tpch-skew0:time}
\shrink
\end{figure}

We have two observations. First, while the running times for most of the queries almost do not change, we can see significant improvement for some queries. For example, as shown in Figure~\ref{fig:tpch-skew0:time:no-calib}, even without calibration of the cost units, the average running time of Q9 drops from 4,446 seconds to only 932 seconds, a 79\% reduction; more significantly, the average running time of Q21 drops from 20,746 seconds (i.e., almost 6 hours) to 3,508 seconds (i.e., less than 1 hour), a 83\% reduction.

Second, calibration of the cost units can sometimes significantly reduce the running times for some queries. For example, comparing Figure~\ref{fig:tpch-skew0:time:no-calib} with Figure~\ref{fig:tpch-skew0:time:calib} we can observe that the average running time of Q8 drops from 3,048 seconds to only 339 seconds, a 89\% reduction, by just using calibrated cost units without even invoking the re-optimization procedure.

\begin{figure}
\centering
\includegraphics[width=\columnwidth]{./figs/reopt-new-join-only-with-dev-skew0-num.eps}
\caption{The number of plans generated during re-optimization over uniform 10GB TPC-H database.}
\label{fig:tpch-skew0:num}
\shrink
\end{figure}

We further studied the re-optimization procedure itself. Figure~\ref{fig:tpch-skew0:num} presents the number of plans generated during re-optimization. It substantiates our observation in Figure~\ref{fig:tpch-skew0:time}: for the queries whose running times were not improved, the re-optimization procedure indeed picked the same plans as those originally chosen by the optimizer. Figure~\ref{fig:tpch-skew0:time-sampling} further compares the query running time excluding/including the time spent on re-optimization. For all the queries we tested, re-optimization time is ignorable compared to query execution time, which demonstrates the low overhead of our re-optimization procedure.

\begin{figure}[t]
\centering
\subfigure[Without calibration of the cost units]{ \label{fig:tpch-skew0:time-sampling:no-calib}
\includegraphics[width=\columnwidth]{./figs/reopt-new-join-only-with-dev-skew0-time-sampling-no-calib.eps}}
\subfigure[With calibration of the cost units]{ \label{fig:tpch-skew0:time-sampling:calib}
\includegraphics[width=\columnwidth]{./figs/reopt-new-join-only-with-dev-skew0-time-sampling-calib.eps}}
\caption{Query running time excluding/including re-optimization time over uniform 10GB TPC-H database ($z=0$).}
\label{fig:tpch-skew0:time-sampling}
\shrink
\end{figure}

\subsubsection{Results on Skewed Database}

On the skewed database, we have observed results similar to that on the uniform database.
%Due to limitation of space, we only present results for the case of $z=1$. Results of $z=2$ (i.e., a more skewed database) are similar and are included in Appendix~\ref{appendix:sec:experiments:tpch-skew2}.
Figure~\ref{fig:tpch-skew1:time} presents the running times of the queries, with or without calibration of the cost units.
While it looks quite similar to Figure~\ref{fig:tpch-skew0:time}, there is one interesting phenomenon not shown before.
In Figure~\ref{fig:tpch-skew1:time:no-calib} we see that, without using calibrated cost units, the average running times for Q8 and Q9 actually increase after re-optimization.
Recall that in Section~\ref{sec:analysis:optimality} (specifically, Theorem~\ref{theorem:local-optimality}) we have shown the local optimality of the plan returned by the re-optimization procedure.
However, that result is based on the assumption that sampling-based cost estimates are consistent with actual costs (Assumption~\ref{assumption:cost-function}).
%\todo{Shall we add some numbers here to show that cardinality estimates are really improved for Q8 and Q9?}
Here this seems not the case.
Nonetheless, after using calibrated cost units, both the running times of Q8 and Q9 were significantly improved (Figure~\ref{fig:tpch-skew1:time:calib}).

\begin{figure}[t]
\centering
\subfigure[Without calibration of the cost units]{ \label{fig:tpch-skew1:time:no-calib}
\includegraphics[width=\columnwidth]{./figs/reopt-new-join-only-with-dev-skew1-time-no-calib.eps}}
\subfigure[With calibration of the cost units]{ \label{fig:tpch-skew1:time:calib}
\includegraphics[width=\columnwidth]{./figs/reopt-new-join-only-with-dev-skew1-time-calib.eps}}
\caption{Query running time over skewed 10GB TPC-H database ($z=1$).}
\label{fig:tpch-skew1:time}
\shrink
\end{figure}

%We also studied the other metrics. Due to space limitations, we include the details in Appendix~\ref{appendix:sec:experiments:tpch-skew1}.
%In summary, the number of plans considered during re-optimization is higher than that on the uniform database, which suggests that re-optimization is more active on skewed data. Meanwhile, the query running times excluding/including the re-optimization times remain almost the same, which implies that the additional overhead of re-optimization is trivial.

\begin{figure}
\centering
\includegraphics[width=\columnwidth]{./figs/reopt-new-join-only-with-dev-skew1-num.eps}
\caption{The number of plans generated during re-optimization over skewed 10GB TPC-H database.}
\label{fig:tpch-skew1:num}
\shrink
\end{figure}

%\begin{figure}
%\centering
%\subfigure[Uniform database with $z=0$]{ \label{fig:tpch:num:skew0}
%\includegraphics[width=\columnwidth]{./figs/reopt-new-join-only-with-dev-skew0-num.eps}}
%\subfigure[Skewed database with $z=1$]{ \label{fig:tpch:num:skew1}
%\includegraphics[width=\columnwidth]{./figs/reopt-new-join-only-with-dev-skew1-num.eps}}
%\subfigure[Skewed database with $z=2$]{ \label{fig:tpch:num:skew2}
%\includegraphics[width=\columnwidth]{./figs/reopt-new-join-only-with-dev-skew2-num.eps}}
%\caption{The number of plans generated during re-optimization over 10GB TPC-H database}
%\label{fig:tpch:num}
%\shrink
%\end{figure}

We further present the number of plans considered during re-optimization in Figure~\ref{fig:tpch-skew1:num}.
Note that re-optimization seems to be more active on skewed data.
Figure~\ref{fig:tpch-skew1:time-sampling} shows the running times excluding/including the re-optimization times of the queries.
Again, the additional overhead of re-optimization is trivial.

\begin{figure}
\centering
\subfigure[Without calibration of the cost units]{ \label{fig:tpch-skew1:time-sampling:no-calib}
\includegraphics[width=\columnwidth]{./figs/reopt-new-join-only-with-dev-skew1-time-sampling-no-calib.eps}}
\subfigure[With calibration of the cost units]{ \label{fig:tpch-skew1:time-sampling:calib}
\includegraphics[width=\columnwidth]{./figs/reopt-new-join-only-with-dev-skew1-time-sampling-calib.eps}}
\caption{Query running time excluding/including re-optimization time over skewed 10GB TPC-H database ($z=1$).}
\label{fig:tpch-skew1:time-sampling}
%\shrink
\vskip -4ex
\end{figure}


\subsubsection{Discussion}

While one might expect the chance for re-optimization to generate a better plan is higher on skewed databases, our experiments show that this may not be the case, at least for TPC-H queries.
There are several different situations, though.
First, if a query is too simple, then there is almost no chance for re-optimization.
For example, Q1 contains no join, whereas Q16 and Q19 involve only one join so only local transformations are possible.
Second, the final plan returned by the re-optimization procedure heavily relies on the initial plan picked by the optimizer, which is the seed or starting point where re-optimization originates.
Note that, even if the optimizer has picked an inefficient plan, re-optimization cannot help if the estimated cost of that plan is not significantly erroneous.
One question is if this is possible: the optimizer picks an inferior plan whose cost estimate is correct?
This actually could happen because the optimizer may (incorrectly) overestimate the costs of the other plans in its search space.
Another subtle point is that the inferior plan might be robust to certain degree of errors in cardinality estimates.
Previous work has reported this phenomenon by noticing that the plan diagram (i.e., all possible plans and their governed optimality areas in the selectivity space) is dominated by just a couple of plans~\cite{Picasso05}.

In summary, the effectiveness of re-optimization depends on factors that are out of the control of the re-optimization procedure itself.
Nevertheless, we have observed intriguing improvement for some long-running queries by applying re-optimization, especially after calibration of the cost units.

\subsection{Results of the Optimizer Torture Test}

We created queries following our design of the OTT in Section~\ref{sec:benchmark:design}.
Specifically, if a query contains $n$ tables (i.e., $n-1$ joins), we let $m$ of the selections be $A=0$ ($A=1$), and let the remaining $n-m$ selections be $A=1$ ($A=0$).
We generated two sets of queries: (1) $n=5$ (4 joins), $m=4$; and (2) $n=6$ (5 joins), $m=4$.
Note that the maximal non-empty sub-queries then contain 3 joins over 4 tables with result size of roughly $100^4=10^8$ rows.\footnote{Recall that a non-empty query must have equal $A$'s (Equation~\ref{eq:non-empty-condition}) and we generated data with roughly 100 rows per distinct value (Section~\ref{sec:experiments:settings}).}
However, the size of each (whole) query is 0.
So we would like to see the ability of the optimizer as well as the re-optimization procedure to identify the empty/non-empty sub-queries.

\begin{figure}[t]
\centering
\subfigure[Without calibration of the cost units]{ \label{fig:hdc-4:time:no-calib}
\includegraphics[width=\columnwidth]{./figs/results-ext-reopt-new-join-only-4-time-no-calib-no-self-joins.eps}}
\subfigure[With calibration of the cost units]{ \label{fig:hdc-4:time:calib}
\includegraphics[width=\columnwidth]{./figs/results-ext-reopt-new-join-only-4-time-calib-no-self-joins.eps}}
\caption{Query running times of 4-join queries.}
\label{fig:hdc-4:time}
\shrink
%\vskip -4ex
\end{figure}

Figure~\ref{fig:hdc-4:time} and~\ref{fig:hdc-5:time} present the running times of the 4-join and 5-join queries, respectively.
We generated in total 10 4-join queries and 30 5-join queries.
Note that the $y$-axes are in log scale and we do not show queries that finish in less than 0.1 second.
As we can see, sometimes the optimizer failed to detect the existence of empty sub-queries: it generated plans where empty join predicates were evaluated after the non-empty ones.
The running times of these queries were then hundreds or even thousands of seconds.
On the other hand, the re-optimization procedure did an almost perfect job in detecting empty joins, which led to very efficient query plans where the empty joins were evaluated first: all the queries after re-optimization finished in less than 1 second.
We also did similar studies regarding the number of plans generated during re-optimization and the time it consumed. Due to space restriction, we include these results in Appendix~\ref{appendix:sec:experiments}.

\begin{figure}[t]
\centering
\subfigure[Without calibration of the cost units]{ \label{fig:hdc-5:time:no-calib}
\includegraphics[width=\columnwidth]{./figs/results-ext-reopt-new-join-only-5-time-no-calib-no-self-joins.eps}}
\subfigure[With calibration of the cost units]{ \label{fig:hdc-5:time:calib}
\includegraphics[width=\columnwidth]{./figs/results-ext-reopt-new-join-only-5-time-calib-no-self-joins.eps}}
\caption{Query running times of 5-join queries.}
\label{fig:hdc-5:time}
\shrink
%\vskip -4ex
\end{figure}

%Quite interestingly, the number of plans generated coincides with the cases where re-optimization indeed identified the empty sub-queries: more plans were attempted during re-optimization.
%Meanwhile, the time spent on re-optimization remains trivial.

%\subsubsection{Discussion}

One might argue that the OTT queries are really contrived: these queries are hardly to see in real-world workloads.
While this might be true, we think these queries serve our purpose as exemplifying extremely hard cases for query optimization.
Note that hard cases are not merely long-running queries: queries as simple as sequentially scanning huge tables are long-running too, but there is nothing query optimization can help with.
Hard cases are queries where efficient execution plans do exist but it might be difficult for the optimizer to find them.
The OTT queries are just these instances.
Based on the experimental results of the OTT queries, re-optimization is helpful to give the optimizer second chances if it initially made a bad decision.

Another concern is if commercial database systems could do a better job on the OTT queries. In regard of this, we also ran the OTT over two major commercial database systems. The performance is very similar to that of PostgreSQL, and we refer readers to Appendix~\ref{appendix:sec:experiments} for the details. We therefore speculate that commercial systems could also benefit from our re-optimization technique proposed in this paper.





==> introduction.tex <==
\section{Introduction}

Cost-based query optimizers rely on reasonable cost estimates of query plans. Cardinality (or selectivity) estimation is crucial for the accuracy of cost estimates. Unfortunately, although decades of research has been devoted to this area and significant progress has been made, cardinality estimation remains challenging in practice. In current database systems, the dominant approach is to keep various statistics about the data, such as histograms, number of distinct values, and list of most common values (MCV). While these statistics can work effectively for estimating selectivities of predicates over a single column, they often fail to accurately estimate selectivities for predicates over multiple columns (e.g., join predicates), especially when data correlation presents.

In our previous work~\cite{WuCHN13,WuCZTHN13,WuWHN14}, we showed that sampling could be used to refine cardinality estimates. However, sampling incurs additional runtime overhead and should be used conservatively. In that line of work, we used sampling for the purpose of making more accurate predictions for query running times, which is efficient because sampling is only used \emph{once} for the final optimal plan that has already been fixed by the query optimizer. In some sense, we used sampling as a way of \emph{validating} optimizer's original cardinality estimates, rather than embedding sampling into the query optimization procedure and using it for every plan considered by the optimizer. Sampling is therefore effective in detecting potential errors in the original cardinality estimates. Nonetheless, if significant errors do exist, the optimality of the ``optimal'' plan is then itself questionable. Given that we have already obtained better cardinality estimates via sampling, would this information help the optimizer generate a better query plan?

In this paper, we present a study of this interesting problem and propose a sampling-based query re-optimization procedure. In a nutshell, our basic idea is as follows: once we have obtained a query plan from the optimizer, we run the plan over samples and obtain refined cardinality estimates; we then let the optimizer know the refined cardinality information and ask it to optimize again. We repeat this process until the optimal plan does not change.

A couple of natural concerns arise regarding this seemingly simple approach. First, is it efficient? As we have just said, sampling should not be abused given its overhead. Since we propose to run plans over samples iteratively, how fast would this procedure converge? To answer this question, we conduct a theoretical analysis as well as an experimental evaluation. Our theoretical study suggests that, in the worst case, the expected number of iterations can be bounded by $O(\sqrt{N})$, where $N$ is the number of plans considered by the optimizer in its search space. In practice, this can rarely happen, though. Re-optimization for most of the queries tested in our experiments converges after only several rounds (most likely only one round) of iteration, and the time spent on re-optimization is ignorable compared with the corresponding query running time.

Second, is it useful? Namely, would re-optimization really generate a better plan? In theory, we can prove that, if the cost model used by the optimizer and the sampling-based cardinality estimates are accurate enough, then the re-optimized plan is guaranteed to be no worse than the original plan. However, cost models are often imperfect, and sampling-based cardinality estimates are imperfect as well. In practice, based on our experimental results, the answer to the above question is: sometimes, but not always. One intriguing example is Q21 of the TPC-H benchmark database. At the scale of 10GB, the running time of the re-optimized plan is about 1 hour while the original plan takes almost 6 hours to finish. For most other TPC-H queries, the re-optimized plans are exactly the same as the original ones. Nonetheless, there are several cases where re-optimized plans are better or worse than original plans. To further evaluate the effectiveness of the re-optimization procedure, we created another benchmark with strong data correlations that are difficult to be detected by existing approaches used by current query optimizers. Our experimental results show the superiority of re-optimized plans over original ones on this benchmark.

Third, is it novel? The idea of query re-optimization can go back to nearly two decades ago~\cite{KabraD98,MarklRSLP04}. The main difference between this line of work and our approach is that re-optimization was previously done \emph{after} a query begins to execute while our re-optimization is done \emph{before} that. While performing re-optimization during the execution of the query has the advantage of being able to observe accurate cardinalities, it suffers from (sometimes significant) runtime overheads such as materializing intermediate results that have been generated in the past period of execution. Meanwhile, runtime re-optimization frameworks usually require significant changes to query optimizer's architecture, such as adding operators that can monitor executions of query plans and adding code that can support switching between query optimization and execution.
Our compile-time re-optimization approach is more lightweight. The only additional cost is due to running tentative query plans over samples. In our experiments, we have observed that this overhead is ignorable compared with query running time. The modification to the query optimizer and executor is also limited. We have implemented our approach in PostgreSQL with only several hundred lines of C code.
%Meanwhile, it can only work for the \emph{rest} of the plan. In other words, the part that has been executed is not revertible.
%Unlike that, our approach is not restricted to partial re-optimization of query plans: it is free to adjust even global join orders.
On the other hand, compile-time re-optimization still relies on imperfect cardinality estimates obtained via sampling while runtime re-optimization can benefit from the true cardinalities.
Furthermore, we should also note that our compile-time re-optimization approach actually does not conflict with these previous runtime re-optimization techniques: the plan returned by our re-optimization procedure could be further refined by using runtime re-optimization. It remains interesting to investigate the effectiveness of this combination framework but it is out of the scope of this paper.

%We discuss the connection between our approach and previous work in more detail in Section~\ref{sec:relatedwork}.

The rest of the paper is organized as follows. We present the details of our iterative sampling-based re-optimization algorithm in Section~\ref{sec:algorithm}. We then present a theoretical analysis of its efficiency in terms of the number of iterations it requires and the quality of the final plan it returns in Section~\ref{sec:analysis}.
To evaluate the effectiveness of this approach, we further present a benchmark database with highly correlated data in Section~\ref{sec:benchmark}, and we report experimental evaluation results on this benchmark as well as the TPC-H benchmark in Section~\ref{sec:experiments}. We discuss related work in Section~\ref{sec:relatedwork} and conclude the paper in~\ref{sec:conclusion}.


==> introductionNew.tex <==
\section{Introduction}

Cost-based query optimizers rely on reasonable cost estimates of query plans. Cardinality (or selectivity) estimation is crucial for the accuracy of cost estimates. Unfortunately, although decades of research has been devoted to this area and significant progress has been made, cardinality estimation remains challenging in practice. In current database systems, the dominant approach is to keep various statistics about the data, such as histograms, number of distinct values, and list of most common values (MCV's).
%\footnote{In this paper we call cardinality estimation approaches that use these statistics ``histogram-based approaches.''}
While these statistics can work effectively for estimating selectivities of predicates over a single column,
%they often fail to accurately estimate selectivities for predicates over multiple columns (e.g., join predicates) or conjunctions of multiple predicates, especially when data correlation presents~\cite{Lohman-critique}.
they can fail to accurately estimate selectivities for conjunctions of multiple predicates, especially when data correlation is present~\cite{Lohman-critique}.

%Sampling-based approaches (e.g.,~\cite{Charikar-sample00,Haas-sample96,Lipton-sample90}) can provide better cardinality estimates on correlated data than histogram-based approaches.
%However, sampling also incurs higher overhead and must be used conservatively.
%In our previous work~\cite{WuCHN13,WuCZTHN13,WuWHN14}, we investigated the effectiveness of using sampling-based cardinality estimates to get better query running time predictions.
%Our key observation in that line of work is the following: rather than using sampling for all, perhaps hundreds of or even thousands of, plans explored by the optimizer during its search for an optimal plan, we use sampling only \emph{once} for the final optimal plan chosen by the optimizer.
%In some sense, we used sampling as a way of \emph{validating} optimizer's original cardinality estimates --- using sampling we can \emph{detect} potential errors in the original estimates.
%Nonetheless, if significant cardinality estimation errors do exist, the optimality of the ``optimal'' plan itself is then also questionable.
%A natural question to ask is then, could the idea of using sampling as a validation step (after the search for an optimal plan is finished) further help the optimizer \emph{correct} the errors and generate a better plan?

%Sampling-based approaches (e.g.,~\cite{Charikar-sample00,Haas-sample96,Lipton-sample90}) can provide
Because sampling-based approaches (e.g.,~\cite{Charikar-sample00,Haas-sample96,Lipton-sample90}) automatically reflect correlation in the data and
between multiple predicates over the data, they can provide better cardinality estimates on correlated data than histogram-based approaches.
However, sampling also incurs higher overhead and must be used conservatively.
In previous work~\cite{WuCHN13,WuCZTHN13,WuWHN14}, the authors investigated the effectiveness of using sampling-based cardinality estimates to get better query running time predictions.
%Our key observation is the following: while it is infeasible to use sampling for all, perhaps hundreds of or even thousands of, plans explored by
The key observation is the following: while it is infeasible to use sampling for all plans explored by
the optimizer during its search for an optimal plan, it is feasible to use sampling as a post-processing step after the search is finished to \emph{detect} potential errors in optimizer's original cardinality estimates for the final chosen plan.

%Nonetheless, if significant cardinality estimation errors do exist, the optimality of the chosen plan itself is then also questionable.
%A natural question to ask is then, could the idea of using sampling as a validation step further help the optimizer \emph{correct} the errors and generate a better plan?

%In this paper, we study the problem of how to use sampling in query optimization without significantly increasing optimization time.
In this paper, we study how to exploit the power of sampling in query optimization without significantly increasing optimization time.
Inspired by the observation that it is feasible to use sampling as a post-processing step to validate cardinality estimates for the final plan returned by the optimizer, our basic idea is simple: if significant cardinality estimation errors are detected, the optimality of the returned plan is then itself questionable, so we go one step further to let the optimizer re-optimize the query by also feeding it the cardinality
estimates refined via sampling.
This gives the optimizer second chance to generate a different, perhaps better, plan.
Note that we can again apply the sampling-based validation step to this new plan returned by the optimizer.
It therefore leads to an iterative procedure based on feedback from sampling: we can repeat this optimization-then-validation loop until the plan chosen by the optimizer does not change.
%In some sense, our approach can be viewed as a compromise between pure histogram-based and pure sampling-based query optimization --- we use
In some sense, our approach can be viewed as a compromise between a histogram-based approach to cardinality estimation and a sampling-based approach --- we use sampling to validate cardinality estimates only for a \emph{subset} (rather than all) of the candidate plans considered by the optimizer and choose the final optimal plan from these validated candidates.
%It is our hope that this re-optimization procedure could catch really big mistakes early in the plans chosen by the optimizer before their execution.
The hope is that this re-optimization procedure can catch large optimizer errors before the system even begins executing the chosen query plan.
%This is in line with the spirit of query optimization: avoid disastrous plans rather than find the real optimal plan.}

%In this paper, we study this interesting problem and propose a sampling-based query re-optimization procedure.
%{\color{blue}Our primary goal is to catch really big mistakes early in the plan (chosen by the optimizer) before its execution.
%This is in line with the spirit of query optimization: avoid disastrous plans rather than find the real optimal plan.}
%The basic idea is as follows: for a given query, once we have obtained a query plan from the optimizer, we run the plan over samples and obtain refined cardinality estimates; we then let the optimizer also know the refined cardinality information and ask it to optimize the query again. If there were significant errors in the original cardinality estimates (by using histogram-based approaches), the optimizer might then generate a different plan. Note that, if this is the case, we can again apply the sampling-based validation step to this new plan.
%It therefore leads to an iterative procedure based on feedback from sampling: we can repeat this optimization-then-validation loop until the optimal plan does not change.
%In a nutshell, our approach can be viewed as a compromise between pure histogram-based and pure sampling-based query optimization --- we use sampling to validate cardinality estimates for a \emph{subset} of the candidate plans considered by the optimizer and choose the final optimal plan from these validated candidates.

A couple of natural concerns arise regarding this simple query re-optimization approach. First, how efficient is it? As we have just said, sampling should not be abused given its overhead. Since we propose to run plans over samples iteratively, how fast does this procedure converge? To answer this question, we conduct a theoretical analysis as well as an experimental evaluation. Our theoretical study suggests that, the expected number of iterations can be bounded by $O(\sqrt{N})$, where $N$ is the number of plans considered by the optimizer in its search space. In practice, this upper bound can rarely happen. Re-optimization for most queries tested in our experiments converges after only a few rounds of iteration, and the time spent on re-optimization is ignorable compared with the corresponding query running time.

Second, is it useful? Namely, does re-optimization really generate a better plan? In theory, we can prove that, if the cost model used by the optimizer and the sampling-based cardinality estimates are accurate enough, then the re-optimized plan is guaranteed to be no worse than the original plan. However, in practice, cost models are often imperfect, and sampling-based cardinality estimates are imperfect as well.
We have implemented our approach in PostgreSQL. Based on experimental results of this implementation, the answer to the above question is: sometimes, but not always. One intriguing example is Q21 of the TPC-H benchmark database. At the scale of 10GB, the running time of the re-optimized plan is about 1 hour while the original plan takes almost 6 hours to finish. For most other TPC-H queries, the re-optimized plans are exactly the same as the original ones. To further evaluate the effectiveness of the re-optimization procedure, we created another database with strong data correlations. %that are difficult to be detected by existing approaches used by current query optimizers.
Not only PostgreSQL but also two commercial RDBMS suffer from major query optimization mistakes on this database.
Given that optimizers have to handle both common cases and difficult, corner cases, our goal is to help cover some of those corner cases. Our experimental results show the superiority of our approach on this database.

%Third, is it novel?
The idea of query re-optimization goes back to two decades ago (e.g.~\cite{KabraD98,MarklRSLP04}). The main difference between this line of work and our approach is that re-optimization was previously done \emph{after} a query begins to execute while our re-optimization is done \emph{before} that. While performing re-optimization during the execution of the query has the advantage of being able to observe accurate cardinalities, it suffers from (sometimes significant) runtime overheads such as materializing intermediate results that have been generated in the past period of execution. Meanwhile, runtime re-optimization frameworks usually require significant changes to query optimizer's architecture, such as adding operators that can monitor executions of query plans and adding code that can support switching between query optimization and execution.
Our compile-time re-optimization approach is more lightweight.
The only additional cost is due to running tentative query plans over samples.
%In our experiments, we have observed that this overhead is ignorable compared with query running time.
The modification to the query optimizer and executor is also limited:
our implementation in PostgreSQL needs only several hundred lines of C code.
%Meanwhile, it can only work for the \emph{rest} of the plan. In other words, the part that has been executed is not revertible.
%Unlike that, our approach is not restricted to partial re-optimization of query plans: it is free to adjust even global join orders.
On the other hand, compile-time re-optimization still relies on imperfect cardinality estimates obtained via sampling while runtime re-optimization can benefit from the true cardinalities.
Furthermore, we should also note that our compile-time re-optimization approach actually does not conflict with these previous runtime re-optimization techniques: the plan returned by our re-optimization procedure could be further refined by using runtime re-optimization. It remains interesting to investigate the effectiveness of this combination framework.
%but it is out of the scope of this paper.

%We discuss the connection between our approach and previous work in more detail in Section~\ref{sec:relatedwork}.

The rest of the paper is organized as follows. We present the details of our iterative sampling-based re-optimization algorithm in Section~\ref{sec:algorithm}. We then present a theoretical analysis of its efficiency in terms of the number of iterations it requires and the quality of the final plan it returns in Section~\ref{sec:analysis}.
To evaluate the effectiveness of this approach, we further design a database (and a set of queries) with highly correlated data in Section~\ref{sec:benchmark}, and we report experimental evaluation results on this database as well as the TPC-H benchmark databases in Section~\ref{sec:experiments}. We discuss related work in Section~\ref{sec:relatedwork} and conclude the paper in Section~\ref{sec:conclusion}.


==> relatedwork.tex <==
\section{Related Work}\label{sec:relatedwork}

Query optimization has been studied for decades, and we refer the readers to~\cite{Chaudhuri98} and~\cite{Ioannidis96} for surveys in this area.

Cardinality estimation is a critical problem in cost-based query optimization, and has triggered extensive research in the database community. Approaches for cardinality estimation in the literature are either static or dynamic.
Static approaches usually rely on various statistics that are collected and maintained periodically in an off-line manner, such as histograms (e.g.,~\cite{Ioannidis-hist03,Poosala-hist97}), samples (e.g.,~\cite{Charikar-sample00,Haas-sample96,Lipton-sample90}), sketches (e.g.,~\cite{Alon-sketch99,Rusu-sketch08}), or even graphical models (e.g.~\cite{GetoorTK01,TzoumasDJ11}). In practice, approaches based on histograms are dominant in the implementations of current query optimizers. However, histogram-based approaches have to rely on the notorious attribute-value-independence (AVI) assumption, and they often fail to capture data correlations, which could result in significant errors in cardinality estimates. While variants of histograms (in particular, multidimensional histograms, e.g.,~\cite{BrunoCG01,MuralikrishnaD88,Poosala-hist97}) have been proposed to overcome the AVI assumption, they are seldom used in real systems, perhaps due to their increasing overhead on large databases.

On the other hand, dynamic approaches further utilize information gathered during query runtime. Approaches in this direction include dynamic query plans (e.g.,~\cite{ColeG94,GraefeW89}), parametric query optimization (e.g.~\cite{IoannidisNSS92}), query feedback (e.g.,~\cite{BrunoC02,Stillger-leo}), mid-query re-optimization (e.g.~\cite{KabraD98,MarklRSLP04}), and quite recently, plan bouquets~\cite{DuttH14}. Dynamic query plans differ from ordinary query plans in that they insert additional ``Choose Plan'' operators~\cite{ColeG94} wherever the optimizer is unsure about the values of some parameters (such as cardinalities). All possible optimal plans are retained and the ``Choose Plan'' operators pick the actual plan at runtime when the true values of the parameters are observed. The idea behind parametric query optimization~\cite{IoannidisNSS92} is similar. For every possible combination of parameter values, the query optimizer generates a plan for a query based on that particular setting. When the query starts, the actual parameter setting is detected and the corresponding plan is used for the execution of the query. Both approaches suffer from the problem of combinatorial explosion and are usually used in contexts where expensive pre-compilation stages are affordable. The recent development of plan bouquets~\cite{DuttH14} is built on top of parametric query optimization so it may also incur a heavy query compilation stage. Unlike standard parametric query optimization that sticks to a single plan at runtime, it chooses a pool of candidate plans and runs them one by one with respect to the increasing order of their estimated costs. While this idea is effective in quickly identifying bad plans that are due to underestimation of their costs, it would increase query running time in general. Therefore, this idea seems to be more attractive if robustness is much more important than average performance.

Meanwhile, approaches based on query feedback record statistics of past queries and use this information to improve cardinality estimates for future queries. Some of these approaches have been adopted in commercial systems such as IBM DB2~\cite{Stillger-leo} and Microsoft SQL Server~\cite{BrunoC02}. Nonetheless, collecting query feedback incurs additional runtime overhead as well as storage overhead of ever-growing volume of statistics. Moreover, the effectiveness of using a mixture of actual/estimated statistics for parts of plans that have/have not been observed in past queries remains debatable. That is, it is unclear if the optimizer could bring up a better plan by giving it partially improved cardinalities. Note that, while our proposed framework faces the same issue, we remedy that by introducing the sampling-based validation stage.

The most relevant work in the literature is the line along mid-query re-optimization~\cite{KabraD98,MarklRSLP04}. We have articulated the connection between our work and this work in the introduction.
%However, previous work performed query re-optimization during the runtime. This decision incurs additional, sometimes significant, overhead such as monitoring query execution and materializing intermediate results. The interleaving between query optimization and execution also requires stopping and resuming query execution frequently, which might be expensive. Unlike these work, our proposed framework re-optimizes queries during the query compilation stage rather than the execution stage. Therefore it is more lightweight. Moreover, in our framework the optimizer is allowed to explore its complete search space freely during re-optimization, while in previous work the optimizer has to consider as well the overhead of the parts of query plans that have been executed. On the other hand, previous re-optimization work can benefit from the true cardinalities while our approach still relies on estimated ones, though, as we have mentioned, the impact of leveraging partially correct cardinalities is not clear.
In some sense, our approach sits between static and dynamic approaches. We combine the advantage of lower overheads from static approaches and the advantage of more optimization opportunities from dynamic approaches. This compromise leads to a lightweight query re-optimization procedure that could bring up better query plans.

Finally, we note that we are not the first that investigates the idea of incorporating sampling into query optimization.
Ilyas et al. proposed using sampling to detect data correlations and then collecting joint statistics for those correlated data columns~\cite{IlyasMHBA04}.
However, this is insufficient if data correlation is caused by specific selection predicates, such as those OTT queries used in our experiments.
Babcock and Chaudhuri also investigated the usage of sampling in developing a robust query optimizer~\cite{BabcockC05}.
While robustness is another interesting goal for query optimizer, it is beyond the scope of this paper. 
